Higher-Order MSL Horn Constraints

The monadic shallow linear (MSL) class is a decidable fragment of first-order Horn clauses that was discovered and rediscovered around the turn of the century, with applications in static analysis and verification. We propose a new class of higher-order Horn constraints which extend MSL to higher-order logic and develop a resolution-based decision procedure. Higher-order MSL Horn constraints can quite naturally capture the complex patterns of call and return that are possible in higher-order programs, which make them well suited to higher-order program verification. In fact, we show that the higher-order MSL satisfiability problem and the HORS model checking problem are interreducible, so that higher-order MSL can be seen as a constraint-based approach to higher-order model checking. Finally, we describe an implementation of our decision procedure and its application to verified socket programming.

==> appx-automata.tex <==
\subsection{Automata}

The following proposition can be generalised to other classes of automata.
The proof hinges on being able to define a subautomaton that checks well-sortedness of a term.
As long as such a subautomaton is definable in a class of automata over ranked trees, the corresponding class of automata over sorted trees is equi-expressive.

In our case, although we consider ATAs, the transitions in the `well-sortedness subautomaton' are ordinary deterministic NFTA transitions.

\eqToNFTA*

\begin{proof}
  First, note that ATAs are no more expressive than NFTAs, \jj{TODO: citation } so it suffices to show that each sorted ATA determines an ordinary ATA and vice versa.

  Any ordinary ATA is a sorted ATA with $Q = Q_\iota$ and first-order alphabet symbols.
  
  For the converse, let $\auto{} = (Q,\Sigma,\_,\transSym)$ be a sorted ATA.
  We construct an equivalent ATA that accepts the same language in two stages:
  \begin{enumerate*}
    \item we `flatten' the sorts of alphabet symbols to first order and\label{stage:flatten}
    \item introduce a `well-sortedness subautomaton' that checks well-sortedness of a term wrt the original sorts. \label{stage:sorted}
  \end{enumerate*} 
  The target ATA shall be $\auto{\prime} = (Q \cup Q_\wellSorted,\Sigma_\flattened,\_,\transSym_\flattened \cup \transSym_\wellSorted)$.
  
  To `flatten' sorts faithfully in stage~\ref{stage:flatten}, we distinguish partial applications by the number of arguments provided;
  for every $f: \sigma_1 \to \dots \to \sigma_m \to \iota \in \Sigma$, we include $f_j : \iota^j \to \iota \in \Sigma_\flattened$, for all $j \in [0..m]$, where arguments $\iota^j$ correspond to $\sigma_1,\dots,\sigma_j$ and tail sort $\iota$ to $\sigma_{j+1} \to \dots \to \sigma_m \to \iota$.
  Formally:
  \begin{align*}
    \Sigma_\flattened     &\defeq \set{ f_j : \iota^j \to \iota \mid f : \sigma_1 \to \dots \to \sigma_m \to \iota \in \Sigma \land j \in [0..m] }
  \end{align*}
  
  Our aim is that if sorted ATA $\auto{}$ accepts a term $t:\sigma$, then ordinary ATA $\auto{\prime}$ accepts the \emph{annotation} $\termAnno{t:\sigma}:\iota$ of this same term:
  \begin{align*}
    \termAnno{f\,t_1 \dots t_j : \sigma} &\defeq f_j\, \termAnno{t_1} \dots \termAnno{t_j}
  \end{align*}
  
  We shall annotate the alphabet symbols in transitions with the number of provided arguments (see $\transSym_\flattened$ below, corresponding to $\transSym$) without subtracting from the structure of the automaton, so it is clear that $\auto{\prime}$ accepts $\termAnno{t}$ if $\auto{}$ accepts $t$.
  However, this may cause the ATA to erroneously accept more than that, because we have lost our well-sortedness guarantee.
  
  For example, consider term $h\,g$ with annotation $h_1\,g_0$.
  The annotation is well-sorted wrt flattened sorts $h_1:\iota \to \iota$ and $g_0 : \iota$, while $h\,g$ itself is not well-sorted wrt the original $h: \iota \to \iota$ and $g: (\iota \to \iota) \to \iota \to \iota$.
  If $\auto{}$ contains a transition $(q,h,\true)$ for some $q \in Q_\iota$ (which is permissible), then $\auto{\prime}$ would contain a transition $(q,h_1,\true)$ and accept $h_1\,g_0$ without checking anything for $g_0$.
  
  To prevent this, in stage~\ref{stage:sorted} we introduce a `well-sortedness subautomaton' that contains a fresh state $q_\sigma$ for all sorts $\sigma \in \sortSet$.
  This subautomaton checks if a term is well-sorted wrt to its original sorts.
  \[
    Q_\wellSorted 
      \defeq \set{ q_\sigma \mid \sigma \in \sortSet }
    \qquad 
    \transSym_\wellSorted 
      \defeq \set{ (q_\sigma, f_j, (q_{\sigma_1},1) \land \dots \land (q_{\sigma_j}, j)) \mid f : \sigma_1 \to \dots \to \sigma_j \to \sigma \in \Sigma }
  \]
  Now, we take the original transitions from $\auto{}$, annotate the input symbols with the number of arguments, and add a conjunct to the `well-sortedness subautomaton' for each argument:
  \[
    \transSym_\flattened 
      \defeq \left\{ 
        (q, f_j, (\theta_1 \land q_{\sigma_1},1) \dots (\theta_j \land q_{\sigma_j},j)) 
          \;\middle|  
        \begin{array}{ll}
           f : \sigma_1 \to \dots \to \sigma_m \to \iota \in \Sigma \land j \in [0..m]  \\
           \;\land\; \left( (\theta_1,1) \land \dots \land (\theta_j,j) \right) \in \transSym(q, f) 
        \end{array} \! \right\}
  \]
  
  In our example, the transition $(q,h,\true)$ in $\auto{}$ becomes $(q,h_1,q_\iota)$ in $\auto{\prime}$.
  However, the only non-false transitions for $g$ are: 
  $(q_{(\iota \to \iota) \to \iota \to \iota}, g_0, \true)$, 
  $(q_{\iota \to \iota}, g_1, (q_{\iota \to \iota}, 1))$, and
  $(q_\iota, g_2, (q_{\iota \to \iota}, 1) \land (q_\iota, 2))$.
  In particular, there exists no $(q_\iota, g_0, \true)$, despite the fact that $g_0: \iota$.

  Claim: term $t'$ over $\Sigma_\flattened$ is accepted by $\auto{\prime}$ from $q_\sigma$ if, and only if, it is an annotation of sort $\sigma$.
  
  We prove this claim by a straightforward induction on terms.
  \begin{itemize}
  
    \item Suppose $t' = f_j \in \Sigma_\flattened$.
      \begin{itemize}
      
        \item For direction $\Rightarrow$, assume $f_j$ is accepted from $q_\sigma$.
          Then, there exists $f : \sigma \in \Sigma$ such that $\transSym_\wellSorted(q_\sigma, f_j) = \true$.
          Thus, $j=0$ and $t' = f_0 = \termAnno{f}$. 
        
        \item For direction $\Leftarrow$, assume $f_j = \termAnno{t}$ for some term $t:\sigma$ over $\Sigma$.
          It must be that $j=0$ and $t = f:\sigma$.
          By construction, $\transSym_\wellSorted(q_\sigma, f_0) = \true$.
          Thus, $t' = f_0$ is accepted from $q_\sigma$.
      
      \end{itemize}
  
    \item Suppose $t' = f\,t_1' \dots t_n'$ over $\Sigma_\flattened$.
     \begin{itemize}
      
        \item For direction $\Rightarrow$, assume $f_j\,t_1' \dots t_n'$ is accepted from $q_\sigma$.
          Then, $j=n$ and there exists $f : \sigma_1 \to \dots \to \sigma_n \to \sigma \in \Sigma$ such that $\transSym_\wellSorted(q_\sigma, f_n) = (q_{\sigma_1},1) \land \dots \land (q_{\sigma_n},n)$ and $t_i$ is accepted from $q_{\sigma_i}$, for all $i \in [1..n]$.
          By the IH, each $t_i' = \termAnno{t_i}$ for some $t_i : \sigma_i$.
          This gives us $t' = f_n\,t_1' \dots t_n' = f_n \, \termAnno{t_1} \dots \termAnno{t_n} = \termAnno{f \, t_1 \dots \,t_n : \sigma}$, as required.
        
        \item For direction $\Leftarrow$, assume $f_j\,t_1' \dots t_n' = \termAnno{t}$ for some term $t:\sigma$ over $\Sigma$.
          It must be that $j=n$ and $t = f\, \termAnno{t_1} \dots \termAnno{t_n}$ for some $f : \sigma_1 \to \dots \to \sigma_n \to \sigma$. 
          Then, $t_i' = \termAnno{t_i : \sigma_i}$, for $i \in [1..n]$.
          By the IH, each $t_i'$ is accepted from $q_{\sigma_i}$.
          By construction, $\transSym_\wellSorted(q_\sigma, f_n) = (q_{\sigma_1},1) \land \dots \land (q_{\sigma_n},n)$ and $f_n \, t_1' \dots t_n'$ is accepted from $q_\sigma$, as required.
      
      \end{itemize}
  
  \end{itemize}

  Now, a simple inductive argument shows that a term $t'$ is accepted by $\auto{\prime}$ from $q \in Q$ if, and only if, there exists $t$ accepted by $\auto{}$ from $q$ such that $t'$ is the annotation of $t$, relying on two observations:
  \begin{enumerate}[label=(\roman*)]

    \item ATA $\auto{\prime}$ only accepts annotations, as per the subproof above.
    
    \item The additional conjuncts in $\transSym_\flattened$ (cf.~$\transSym$) ensure $\auto{\prime}$ can never accept more than %(the annotations of terms accepted by) 
      $\auto{}$. 

  \end{enumerate}

   The ordinary ATA $\auto{\prime} = (Q \cup Q_\wellSorted,\Sigma_\flattened,\_,\transSym_\flattened \cup \transSym_\wellSorted)$ now defines the same language as sorted ATA $\auto{} = (Q,\Sigma,\_,\transSym)$ (up to the annotation, which is easily undone).
  %\jj{The annotation can be undone easily (invoke reflectivity, at most), so this is in fact the same language.}

\end{proof}

\begin{lemma}
  \label{lem:aux_subsumption}
  \begin{enumerate}[label=(\roman*)]
    \item If $\apath{q'}{\epsilon}{q}$ in $\auto{}$, then $\apath{\set{q}}{\epsilon}{\set{q'}}$ in $\sauto{}$ through singleton states. \label{enum:eps_reverse}
    \item If $\apath{\set{q}}{\epsilon}{\set{q'}}$ through singleton states and $\apath{S}{\epsilon}{S'}$ in $\sauto{}$, then $\apath{S \cup \set{q}}{\epsilon}{S' \cup \set{q'}}$ in $\sauto{}$. \label{enum:eps_union}
  \end{enumerate}
\end{lemma}
\begin{proof}
  We prove~\ref{enum:eps_reverse} by a straightforward induction on length $n$ of the path.
  Base case $n=0$ is trivial, so suppose $q'' \xrightarrow{\epsilon} q' \mathbin{\xrightarrow{\epsilon}}^n q$.    
  For every transition $(q'',\epsilon,q')$ in $\auto{}$, subsumption automaton $\sauto{}$ contains a transition $(\set{q'},\epsilon,\set{q''})$ (see Definition~\ref{def:prod_subsumption_auto}).
  By the IH, $\apath{\set{q}}{\epsilon}{\set{q'}}$.
  Finally, transitivity gives us $\apath{\set{q}}{\epsilon}{\set{q''}}$.
    
  For~\ref{enum:eps_union}, we use an outer induction on the length $m$ of $\apath{S}{\epsilon}{S''}$ and an inner induction on length $n$ of $\apath{\set{q}}{\epsilon}{\set{q''}}$ in $\sauto{}$. 
  \begin{itemize}
    \item \textbf{Base case $m=0$.} The subcase where $n=0$ follows from $S \cup \set{q} \in \statesA{\sauto{}}$, so suppose $\set{q} \xrightarrow{\epsilon} \set{q'} \mathbin{\xrightarrow{\epsilon}}^n \set{q''}$.
      By the IH, $\apath{S \cup \set{q'}}{\epsilon}{S \cup \set{q''}}$.
      Note that $\set{q} \xrightarrow{\epsilon} \set{q'}$ can only be inherited from $(q',\epsilon,q)$ in $\auto{}$.
      If $q \in S$, then we have a path $S \cup \set{q} \xrightarrow{\epsilon} S \backslash \set{q} \cup \set{q'} \xrightarrow{\epsilon} S \cup \set{q'}$ using an inclusion-transition.
      Otherwise, if $q \not\in S$, then $S \cup \set{q} \xrightarrow{\epsilon} S \cup \set{q'}$.
      
    \item \textbf{Case $m>0$.} Suppose $S \xrightarrow{\epsilon} S' \xrightarrow{\epsilon}^m S''$.
      Suppose $n=0$.
      By the IH, $\apath{S' \cup \set{q}}{\epsilon}{S'' \cup \set{q}}$.
      If $S \xrightarrow{\epsilon} S'$ is an inclusion-transition, there also exists an inclusion-transition $S \cup \set{q} \xrightarrow{\epsilon} S' \cup \set{q}$.
      Otherwise, there exists $(q_2,\epsilon,q_1)$ in $\auto{}$ such that $q_1 \in S$ and $S' = S \backslash \set{q_1} \cup \set{q_2}$.
      If $q = q_1$, then there exists $S \cup \set{q} \xrightarrow{\epsilon} S \backslash \set{q_1} \cup \set{q_2} \xrightarrow{\epsilon} S' \cup \set{q}$ using an inclusion-transition.
      Otherwise, if $q \neq q_1$, then $S \cup \set{q} \xrightarrow{\epsilon} S' \cup \set{q}$ with the same $(q_2,\epsilon,q_1)$ as side-condition.
      Transitivity gives us $\apath{S \cup \set{q}}{\epsilon}{S'' \cup \set{q}}$.
    
      Finally, suppose $\set{q} \xrightarrow{\epsilon} \set{q'} \mathbin{\xrightarrow{\epsilon}}^n \set{q''}$.
      By the IH on $m$, $\apath{S \cup \set{q}}{\epsilon}{S \cup \set{q''}}$.
      Furthermore, by the IH on $n$, $\apath{S \cup \set{q''}}{\epsilon}{S'' \cup \set{q''}}$.
      Transitivity concludes this case and the proof.   
      
  \end{itemize}

\end{proof}

\corrSubsumptionAutomata*

\begin{proof}

  We first prove direction $\Leftarrow$ by structural induction on typing proofs.

  \textbf{\ruleName{Q-Bas}}.
  Suppose $q \leq q'$ with $(q,q') \in \preorder$.
  Our intersection types are derived from automaton clauses as per Definition~\ref{def:HOMSL_intersection_type_correspondence}.
  Therefore, preorder $\preorder$ is merely the identity on base types $\basetypes$ and $q=q'$.
  Trivially, $\apath{q}{\epsilon}{q}$ for all $q \in \statesA{\auto{\iota}}$.

  \textbf{\ruleName{Q-Prj}}.
  Suppose $\bigwedge_{j=1}^n \tau_j \leq \tau_i$ for some $i \in [1..n]$.
  Trivially, $\apath{\tau_i}{\epsilon}{\tau_i}$.
  
  \textbf{\ruleName{Q-Glb}}.
  This case is immediate from the IH.

  \textbf{\ruleName{Q-Trs}}.
  Suppose $\theta \leq \tau$ of sort $\sigma$ with $\theta \leq \theta'$ and $\theta' \leq \tau$.
  We obtain the existence of $\tau' \in \theta'$ such that $\apath{\tau}{\epsilon}{\tau'}$ in $\auto{\sigma}$ from the IH.
  Furthermore, there exists $\tau'' \in \theta$ such that such that $\apath{\tau'}{\epsilon}{\tau''}$, which gives us $\apath{\tau}{\epsilon}{\tau''}$ by transitivity.

  \textbf{\ruleName{Q-Arr}}.
  Suppose $\bigwedge_{j=1}^m \tau_j' \to \tau_1 \leq \bigwedge_{i=1}^n \tau_i \to \tau_2$ of sort $\sigma \to \sigma'$ with $\bigwedge_{i=1}^n \tau_i \leq \bigwedge_{j=1}^m \tau_j'$ and $\tau_1 \leq \tau_2$.
  By the IH, $\apath{\tau_2}{\epsilon}{\tau_1}$ in $\auto{\sigma'}$.
  Lemma~\ref{lem:subtyping} gives us $\forall j \in [1..m].\,\exists i_j \in [1..n].\, \tau_{i_j} \leq \tau_j'$.
  Again, by the IH, $\forall j \in [1..m].\,\exists i_j \in [1..n].\, \apath{\tau_j'}{\epsilon}{\tau_{i_j}}$ in $\auto{\sigma}$. 
  (This use of the IH is justified by each $\tau_{i_j} \leq \tau_j'$ being a subproof of $\bigwedge_{i=1}^n \tau_i \leq \bigwedge_{j=1}^m \tau_j'$.)
  Lemma~\ref{lem:aux_subsumption} gives us $\apath{\bigwedge_{j=1}^m \tau_{i_j}}{\epsilon}{\bigwedge_{j=1}^m \tau_j'}$.
  Subsumption automaton $\sauto{\sigma}$ contains an inclusion-transition $\apath{\bigwedge_{i=1}^n \tau_i}{\epsilon}{\bigwedge_{j=1}^m \tau_{i_j}}$, because $\set{\tau_{i_1},\dots,\tau_{i_m}} \subseteq \set{\tau_1,\dots,\tau_n}$.
  Transitivity gives us $\apath{\bigwedge_{i=1}^n \tau_i}{\epsilon}{\bigwedge_{j=1}^m \tau_j'}$.
  Finally, product automaton $\auto{\sigma \to \sigma'} = \sauto{\sigma} \times \auto{\sigma}$ runs $\apath{\bigwedge_{i=1}^n \tau_i}{\epsilon}{\bigwedge_{j=1}^m \tau_j'}$ in $\sauto{\sigma}$ in parallel with $\apath{\tau_2}{\epsilon}{\tau_1}$ in $\auto{\sigma'}$ as $\apath{\left( \bigwedge_{i=1}^n \tau_i \to \tau_2 \right)}{\epsilon}{\left( \bigwedge_{j=1}^m \tau_j' \to \tau_1 \right)}$ in $\auto{\sigma \to \sigma'}$, which concludes this case.

  \textbf{\ruleName{Q-Fun}}.
  Suppose $\bigwedge_{i=1}^n (\sigmaInt \to \tau_i) \leq \sigmaInt \to \tau$ of sort $\sigma \to \sigma'$ with $\bigwedge_{i=1}^n \tau_i \leq \tau$.
  By the IH, there exists $j \in [1..n]$ such that $\apath{\tau}{\epsilon}{\tau_j}$ in $\auto{\sigma'}$.
  Trivially, $\apath{\sigmaInt}{\epsilon}{\sigmaInt}$ in $\sauto{\sigma}$.
  We combine this to $\apath{(\sigmaInt \to \tau)}{\epsilon}{(\sigmaInt \to \tau_j)}$ in $\auto{\sigma \to \sigma'} = \sauto{\sigma} \times \auto{\sigma'}$, as required.
  
  For direction $\Rightarrow$, it suffices to show that $\apath{\tau}{\epsilon}{\tau'}$ implies $\tau' \leq \tau$.
  To see why, first observe that the following statements are equivalent (for implicitly universally quantified variables):
  \[
    (\apath{\tau}{\epsilon}{\tau'} \land \tau' \in \theta) \Rightarrow \theta \leq \tau 
      \qquad\iff\qquad
    \apath{\tau}{\epsilon}{\tau'} \Rightarrow \tau' \in \theta \Rightarrow \theta \leq \tau
  \]
  Second, note that $\tau' \leq \tau$ implies $\forall \theta.\, \tau' \in \theta \Rightarrow \theta \leq \tau$ thanks to \ruleName{Q-Prj} and \ruleName{Q-Trs}.
  Furthermore, we can restrict ourselves to single $\epsilon$-transitions: if $\tau \xrightarrow{\epsilon} \tau'$ in $\auto{\sigma}$, then $\tau' \leq \tau$.
  
  The case where $\sigma = \iota$ is immediate from $\auto{\iota}$ containing no $\epsilon$-transitions, so suppose $\sigma = \sigma' \to \sigma''$.
  
  Suppose $(\sigmaInt_1 \to \tau_1) \xrightarrow{\epsilon} (\sigmaInt_2 \to \tau_2)$ in $\auto{\sigma' \to \sigma''} = \sauto{\sigma'} \times \auto{\sigma''}$.
  This means that $\sigmaInt_1 \xrightarrow{\epsilon} \sigmaInt_2$ in $\sauto{\sigma'}$ and $\tau_1 \xrightarrow{\epsilon} \tau_2$ in $\auto{\sigma''}$.
  By the IH, $\tau_2 \leq \tau_1$.
  We distinguish two subcases for $\sigmaInt_1 \xrightarrow{\epsilon} \sigmaInt_2$ in $\sauto{\sigma'}$:
  \begin{itemize}
  
    \item \textbf{Inclusion-transition.}
      In this case, $\sigmaInt_2 \subseteq \sigmaInt_1$, which means $\sigmaInt_1 \leq \sigmaInt_2$.
    
    \item \textbf{Inherited transition.} 
      There exists $(\tau'',\epsilon,\tau')$ in $\auto{\sigma'}$ such that $\sigmaInt_2 = \sigmaInt_1 \backslash \set{\tau'} \cup \set{\tau''}$ with $\tau' \in \sigmaInt_1$.
      By the IH, $\tau' \leq \tau''$.
      We prove $\sigmaInt_1 \leq \sigmaInt_2$ in the following way.
      (Unfinished branches denote known facts.)
      \[
        \prftree[l]
        { \ruleName{Q-Glb} }
          {{\prftree[l]
              { \ruleName{Q-Prj} }
              {\forall \tau''' \in \sigmaInt_1 \backslash \set{\tau'}.\; \sigmaInt_1 \leq \tau'''}
           }}
          {\prftree[l]
            { \ruleName{Q-Trs} }
            {{\prftree[l]
              { \ruleName{Q-Prj} }
              {\sigmaInt_1 \leq \tau'}
            }}
            {\tau' \leq \tau''}
            {\sigmaInt_1 \leq \tau''}
          }
        {\sigmaInt_1 \leq \sigmaInt_1 \backslash \set{\tau'} \cup \set{\tau''}}
      \]
      Finally, \ruleName{Q-Arr} derives $(\sigmaInt_2 \to \tau_2) \leq (\sigmaInt_1 \to \tau_1)$ from $\sigmaInt_1 \leq \sigmaInt_2$ and $\tau_2 \leq \tau_1$.
      
  \end{itemize}
\end{proof}

\begin{lemma}
  \label{lem:subsumption_for_intersections}
  If $\parEps{[\theta_1,\dots,\theta_m]}{[\theta'_1,\dots,\theta'_m]}$, then $\theta_i' \leq \theta_i$ for all $i\in [1..m]$.
\end{lemma}
\begin{proof}
  By definition of parallel $\epsilon$-run-trees, it suffices to prove the claim for $m=1$.

  Suppose $\parEps{[\theta]}{[\theta']}$. 
  Let $\theta = \bigwedge_{j=1}^k \tau_j$ and $\theta' = \bigwedge_{i=1}^n \tau_i'$.
  
  By definition, assumption $\parEps{[\bigwedge_{j=1}^k \tau_j]}{[\bigwedge_{i=1}^n \tau_i']}$ requires $\forall j \in [1..k].\,\exists i_j \in [1..n].\, \atree{\tau_j}{\epsilon}{\tau'_{i_j}}{1}$. % and $\set{\tau_1',\dots,\tau'_n} = \set{\tau'_{i_1},\dots,\tau'_{i_k}}$.
  Lemma~\ref{lem:correctness_subsumption_automaton} gives us $\theta' \leq \tau_j$, for all $j \in [1..k]$.
  Finally, subtyping rule \ruleName{Q-Glb} yields $\theta' \leq \theta$.

\end{proof}

  Note that an intersection type in a run-tree corresponds to a conjunction of branches (i.e.~of strict types). 
  Intuitively, the above consequences of $\theta_i \leq \theta_i''$ prove there exist $\epsilon$-paths from (the branches of) $\theta_i''$ to a subset of (the branches of) $\theta_i$.
  We also have $\theta_i' \subseteq \theta_i''$, which means there exist $\epsilon$-paths from (the branches of) $\theta_i'$ to an even smaller subset of (the branches of) $\theta_i$, by transitivity.

\begin{lemma}
  \label{lem:parEps}
  If $\sigmaInt \leq \sigmaInt'$, then there exists $\sigmaInt'' \subseteq \sigmaInt$ such that $\parEps{[\sigmaInt']}{[\sigmaInt'']}$.
\end{lemma}
\begin{proof}
  Suppose $\bigwedge_{i=1}^{n} \tau_{k} \leq \bigwedge_{j=1}^{m} \tau_{j}'$.
  By Lemma~\ref{lem:subtyping}, for every $j \in [1..m]$, there exists $i_j \in [1..n]$ such that $\tau_{i_j} \leq \tau_{j}'$.
  Lemma~\ref{lem:correctness_subsumption_automaton} gives us $\atree{\tau_{j}'}{\epsilon}{[\tau_{i_j}]}{1}$, for all $j \in [1..m]$, which yields $\parEps{[\bigwedge_{j=1}^{m} \tau_{j}']}{[\bigwedge_{j=1}^{m} \tau_{i_j}]}$, where $\bigwedge_{j=1}^{m} \tau_{i_j} \subseteq \bigwedge_{i=1}^{n} \tau_{k}$. 
\end{proof}

\corrTypeCheckingAutomaton*

\begin{proof}
  By construction, type-checking automaton $\auto{V}$ captures subtyping within each sort-partition;
  there exists a path $\apath{\tau_2}{\epsilon}{\tau_1}$ in $\auto{V}$ if and only if $\tau_1 \leq \tau_2$, for all relevant sorts (see Lemma~\ref{lem:correctness_subsumption_automaton}).
  
  We use structural induction on terms to prove that $\auto{V}$ captures typing for all terms $t$.

  Suppose $t = f \in \Sigma$.
  
  For direction $\Leftarrow$, assume $\atree{\tau}{f}{[\theta_1',\dots,\theta_m']}{m}$ in $\auto{V}$ with $\theta_i' \subseteq \theta_i$, for all $i \in [1..m]$.
  An inclusion $\theta_i' \subseteq \theta_i$ implies $\theta_i \leq \theta_i'$, by \ruleName{Q-Prj} and \ruleName{Q-Glb}.
  Now, \ruleName{Q-Arr} proves $\theta_1' \to \dots \to \theta_m' \to \tau \leq \theta_1 \to \dots \to \theta_m \to \tau$.
  
  Any run-tree on $f$ contains a single $f$-labelled transition and any number of $\epsilon$-transitions, so our run-tree decomposes as $\atree{\tau}{\epsilon}{[\tau']}{1}$ and $\atree{\tau'}{f}{[\theta_1'',\dots,\theta_m'']}{m}$ and $\parEps{[\theta_1'',\dots,\theta_m'']}{[\theta_1',\dots,\theta_m']}$ for some transition $(\theta_1'',1) \land \dots \land (\theta_m'',m) \in \transSet{V}(\tau',f)$ such that $\theta_1'' \to \dots \to \theta_m'' \to \tau' \in \fromClause{\res{V}{f}}$.
  Note that $\fromClause{\res{V}{f}} \leq \theta_1'' \to \dots \to \theta_m'' \to \tau'$ by \ruleName{Q-Prj}.
  
  By Lemma~\ref{lem:correctness_subsumption_automaton} and~\ref{lem:subsumption_for_intersections}, $\tau' \leq \tau$ and $\theta_i' \leq \theta_i''$, for all $i \in [1..m]$.
  It follows from subtyping rule \ruleName{Q-Arr} that $\theta_1'' \to \dots \to \theta_m'' \to \tau' \leq \theta_1' \to \dots \to \theta_m' \to \tau$.
  
  Rule \ruleName{Q-Trs} now gives us $\typeSet{f} = \fromClause{\res{V}{f}} \leq \theta_1 \to \dots \to \theta_m \to \tau$, as required.
   
  For direction $\Rightarrow$, assume $\typeSet{t} \leq \theta_1 \to \dots \to \theta_m \to \tau$, so $\fromClause{\res{V}{f}} \leq \theta_1 \to \dots \to \theta_m \to \tau$ and there exists $\theta_1' \to \dots \to \theta_m' \to \tau' \in \fromClause{\res{V}{f}}$ such that $\theta_1' \to \dots \to \theta_m' \to \tau' \leq \theta_1 \to \dots \to \theta_m \to \tau$, by Lemma~\ref{lem:subtyping}.
  Thus, $\tau' \leq \tau$ and $\theta_i \leq \theta_i'$, for all $i \in [1..m]$.
  By Lemma~\ref{lem:correctness_subsumption_automaton}, $\atree{\tau}{\epsilon}{[\tau']}{1}$.
  
  By construction, $(\theta_1',1) \land \dots \land (\theta_m',m) \in \transSet{V}(\tau',f)$.
  Thus, there exists a run-tree $\atree{\tau'}{f}{[\theta_1',\dots,\theta_m']}{m}$ that composes into $\atree{\tau}{f}{[\theta_1',\dots,\theta_m']}{m}$ with $\atree{\tau}{\epsilon}{[\tau']}{1}$.
  Lemma~\ref{lem:parEps} derives $\parEps{[\theta_i']}{[\theta_i'']}$ from $\theta_i \leq \theta_i'$ for some $\theta_i'' \subseteq \theta_i'$, which we compose with $\atree{\tau}{f}{[\theta_1',\dots,\theta_m']}{m}$ for $\atree{\tau}{f}{[\theta_1'',\dots,\theta_m'']}{m}$ to prove this case.
  
  Suppose $t = s\,t'$ for terms $s : \sigma' \to \sigma_1 \to \dots \to \sigma_m \to \sigma$ and $t': \sigma'$.
  
  For direction $\Leftarrow$, assume $\atree{\tau}{s\,t'}{[\theta_1',\dots,\theta_m']}{m}$ in $\auto{V}$ with $\theta_i' \subseteq \theta_i$, for all $i \in [1..m]$.
  There exists a type $\sigmaInt = \bigwedge_{j=1}^n \tau_j' : \sigma'$ such that $\atree{\tau}{s\,t'}{[\theta_1',\dots,\theta_m']}{m}$ decomposes into $\atree{\tau}{s}{[\sigmaInt,\theta_1',\dots,\theta_m']}{m+1}$ and $\atree{\tau_j'}{t'}{[]}{0}$, for all $j \in [1..n]$.
  
  By the IH, $\typeSet{s} \leq \sigmaInt \to \theta_1' \to \dots \to \theta_m' \to \tau$ and $\typeSet{t'} \leq \tau_j'$, for all $j \in [1..n]$.
  Subtyping rule \ruleName{Q-Glb} gives us $\typeSet{t'} \leq \sigmaInt$, and Lemma~\ref{lem:subtyping} the existence of $\sigmaInt' \to \theta_1'' \to \dots \to \theta_m'' \to \tau' \in \typeSet{s}$ such that $\sigmaInt' \to \theta_1'' \to \dots \to \theta_m'' \to \tau' \leq \sigmaInt \to \theta_1' \to \dots \to \theta_m' \to \tau$.
  This means that $\sigmaInt \leq \sigmaInt'$ and $\tau' \leq \tau$ and $\theta_i' \leq \theta_i''$, for all $i \in [1..m]$.
   
  It follows from $\sigmaInt' \to \theta_1'' \to \dots \to \theta_m'' \to \tau' \in \typeSet{s}$ and $\typeSet{t'} \leq \sigmaInt \leq \sigmaInt'$ that $\theta_1'' \to \dots \to \theta_m'' \to \tau' \in \typeSet{s\,t'}$.
  Thus, $\typeSet{s\,t'} \leq \theta_1' \to \dots \to \theta_m' \to \tau$.
  Since we assumed $\theta_i' \subseteq \theta_i$, also $\theta_i \leq \theta_i'$ and $\theta_1' \to \dots \to \theta_m' \to \tau \leq \theta_1 \to \dots \to \theta_m \to \tau$.
  
  Finally, transitivity gives us $\typeSet{s\,t'} \leq \theta_1 \to \dots \to \theta_m \to \tau$.
     
  For direction $\Rightarrow$, assume $\typeSet{s\,t'} \leq \theta_1 \to \dots \to \theta_m \to \tau$.
  There exists $\theta_1'' \to \dots \to \theta''_m \to \tau'' \in \typeSet{s\,t'}$ such that $\theta_1'' \to \dots \to \theta''_m \to \tau'' \leq \theta_1 \to \dots \to \theta_m \to \tau$, by Lemma~\ref{lem:subtyping}.
  This means there exists $\sigmaInt : \sigma'$ such that $\sigmaInt \to \theta_1'' \to \dots \to \theta''_m \to \tau'' \in \typeSet{s}$ and $\typeSet{t'} \leq \sigmaInt$.
  We can apply to IH to the former (thanks to \ruleName{Q-Prj}) for run-tree $\atree{\tau''}{s}{[\theta_0',\theta_1',\dots,\theta_m']}{m+1}$ for some $\theta_0' \subseteq \sigmaInt$ and $\theta_i' \subseteq \theta_i''$, for all $i \in [1..m]$.
      
  Let $\sigmaInt = \bigwedge_{j=1}^n \tau_j$.      
  Subtyping rules \ruleName{Q-Prj} and \ruleName{Q-Trs} give us $\forall j \in [1..n].\, \typeSet{t'} \leq \tau_j$.
  By the IH, there exists a run-tree $\atree{\tau_j}{t'}{[]}{0}$, for all $j \in [1..n]$.      
  Now, because $\theta_0' \subseteq \sigmaInt$, there exists an accepting run-tree $\atree{\tau_0'}{t'}{[]}{0}$ for every strict type $\tau_0' \in \theta_0'$, giving rise to a composed run-tree $\atree{\tau''}{s\,t'}{[\theta_1',\dots,\theta_m']}{m}$.
  
  We know from $\theta_1'' \to \dots \to \theta''_m \to \tau'' \leq \theta_1 \to \dots \to \theta_m \to \tau$ that $\tau'' \leq \tau$ and $\theta_i \leq \theta_i''$, for all $i \in [1..m]$.  
  By Lemma~\ref{lem:correctness_subsumption_automaton}, we have a run-tree $\atree{\tau}{\epsilon}{\tau''}{1}$ and, thus, a composed run-tree $\atree{\tau}{s\,t'}{[\theta_1',\dots,\theta_m']}{m}$.
  Lemma~\ref{lem:parEps} derives $\parEps{[\theta_i'']}{[\theta_i''']}$ from $\theta_i \leq \theta_i''$ for some $\theta_i''' \subseteq \theta_i$.
  Furthermore, because $\theta_i' \subseteq \theta_i''$, there exists an even smaller $\theta^{(4)}_i \subseteq \theta_i''' \subseteq \theta_i$ such that $\parEps{[\theta_i']}{[\theta^{(4)}_i]}$.
 
  Finally, we compose these simultaneous run-trees with $\atree{\tau}{s\,t'}{[\theta_1',\dots,\theta_m']}{m}$ for $\atree{\tau}{s\,t'}{[\theta^{(4)}_1,\dots,\theta^{(4)}_m]}{m}$, which proves the claim along with $\theta^{(4)}_i \subseteq \theta_i$, for all $i \in [1..m]$.

\end{proof}

==> appx-semantic_correspondence.tex <==
\subsection{Semantic correspondence with HOCHC}

\newcommand\asem[1]{\calA^\omega\sem{#1}}
\newcommand\hframe{\calA^\mathrm{Th}}
\newcommand\hsem[1]{\hframe\sem{#1}}
\newcommand\upTo[2]{\calA^{{#1}\,\uparrow}_{#2}}
\newcommand\downTo[2]{\calA^{{#1}\,\downarrow}_{#2}}
\newcommand\upToMSL[1]{\upTo{\omega}{#1}}
\newcommand\downToMSL[1]{\downTo{\omega}{#1}}
\newcommand\upToH[1]{\upTo{\mathrm{Th}}{#1}}
\newcommand\downToH[1]{\downTo{\mathrm{Th}}{#1}}
\newcommand\topOf[1]{\top_{#1}}
\newcommand\botOf[1]{\bot_{#1}}
\newcommand\id{\mathsf{id}}
\newcommand\qmH[1]{\precsim_{#1}^{\mathrm{Th}}}
\newcommand\qmMSL[1]{\precsim_{#1}^{\omega}}
\newcommand\qm{\precsim}
\newcommand\lub{\bigsqcup}
\newcommand\canMod{\alpha_{\mathrm{can}}}

\jj{TODO above:
  \begin{itemize}
    \item $\rho$ should be $\trSem{\rho}$ in elim of predicate-type existentials
  \end{itemize}
}

\subsubsection{Domain theory}

We add a fictitious smallest tree $\bot$ and largest tree $\top$ to $\asem{\iota}$ and $\hsem{\iota}$ while maintaining the discrete orderings.

\begin{lemma}
  Each $\asem{\gamma}$ is a discretely ordered dcpo wrt $\sqsubseteq$. \jj{DONE}
\end{lemma}
%\begin{proof}
%  Recall that $\asem{\iota}$ is discretely ordered by definition. 
%  Consider type $\gamma_1 \to \gamma_2$.
%  Let $f,g \in \asem{\gamma_1 \to \gamma_2}$.
%  The following sequence of equivalences holds:
%  \begin{align*}
%    f \sqsubseteq g 
%      &\iff \forall e \in \asem{\gamma_1}.\, f\,e \sqsubseteq g\,e \\
%      &\iff \forall e \in \asem{\gamma_1}.\, f\,e = g\,e \qquad \text{by IH on } \gamma_2 \\
%      &\iff f = g
%  \end{align*}
%  
%  Now, the only directed sets in a discretely ordered poset are singleton sets;
%  the single element in such a directed set is the least upper bound of this set, so each $\asem{\gamma}$ is a dcpo.
%\end{proof}

\begin{lemma}
  Each $\asem{\rho}$ is a complete lattice wrt $\sqsubseteq$.
\end{lemma}
\begin{proof}
  By definition, \changed[jj]{provided the frame $\calA$ is complete.}
\end{proof}

The corresponding results for $\hsem{\trSem{\sigma}}$ are inherited from \cite{OngWagner2019}.


\subsubsection{Quasi-monotonicity}

\begin{definition}[Quasi-monotonicity]
  A function is \emph{quasi-monotone} if it acts monotonically on quasi-monotone inputs.
  Formally, we adapt the order from \cite{OngWagner2019}'s Definition 19 to $\qmH{\sigma}$ and define an MSL counterpart $\qmMSL{\sigma}$ through:
  \begin{align*}
    n \qmMSL{\iota} n' & \defeq n = n' \lor n = \bot \lor n' = \top \\%\exists t:\iota.\, \asem{t} = n = n'\\
    b \qmMSL{o} b' & \defeq b \sqsubseteq_o b' \\
    r \qmMSL{\sigma_1 \to \sigma_2} r' & \defeq \forall s,s' \in \asem{\sigma_1}.\, s \qmMSL{\sigma_1} s' \Rightarrow r\,s \qmMSL{\sigma_2} r'\,s'
  \end{align*}
  The order $\qmH{\sigma}$ is defined analogously.
  
  We omit the subscript and superscript of $\qm$ when it is clear from the context, allowing us to say a function $F: A \to B$ (with $A$ and $B$ ordered wrt some $\qm$) is quasi-monotone just if $F\,a \qm F\,a'$ for all $a,a' \in A$ such that $a \qm a'$.
  Note: this is equivalent to saying that $F$ is quasi-monotone just if $F \qm F$.
\end{definition}

%\jj{We probably need to tweak the definition of $\qmMSL{\iota}$ to account for $\bot$ and $\top$ being the smallest and largest tree, resp.
%Let us try $n \qmMSL{\iota} n'  \defeq n = n' \lor n = \bot \lor n' = \top$.
%  \begin{enumerate}
%    \item $\asem{\iota}$ is the set of trees + $\bot$
%    \item $\asem{\iota}$ is the set of trees + $\bot$ + $\top$
%    \item $\asem{\iota}$ is the set of trees + $\top$
%    \item $\asem{\iota}$ is the set of trees + $\bot$ with $\bot \sqsubseteq t$
%  \end{enumerate}
%  We could also say $\bot$ is less in $\lesssim$ but not $\sqsubseteq$, but that prob becomes incompatible with the discretely ordered HOCHC poset.
%}

%\jj{We must include $\bot$ in the criterion of quasi-monotonicity.}

\begin{definition}[Compatibility criteria]
  According to Definition 16 from \cite{OngWagner2019}, $\qmMSL{\sigma}$ is compatible with $\sqsubseteq$ on $\asem{\sigma}$ if:
  \begin{enumerate}
    \item for all $a,b,c \in \asem{\sigma}$, if $a \qmMSL{\sigma} b$ and $b \sqsubseteq c$, then $a \qmMSL{\sigma} c$ \label{comp:trans}
    \item for all $a \in \asem{\sigma}$ and $A \subseteq \set{b \in \asem{\sigma} \mid b \qmMSL{\sigma} a}$, $\bigsqcup A \qmMSL{\sigma} a$ \changed[jj]{if $\bigsqcup A$ exists in $\asem{\sigma}$} \label{comp:lub}
  \end{enumerate}
  Compatibility of $\qmH{\trSem{\sigma}}$ with $\sqsubseteq$ on $\hsem{\trSem{\sigma}}$ is defined analogously.
\end{definition}

\begin{lemma}
  Each $\qmMSL{\rho}$ is compatible with $\sqsubseteq$ on $\asem{\rho}$. \jj{DONE}
\end{lemma}
%\begin{proof}
%  
%  %\jj{We could qualify this second requirement with ``if the lub exists in the set''.}
%  
%  This is immediate for type $o$, % and $\iota$ \jj{(pending the choice of $\asem{\iota}$)}.
%  so consider $\sigma \to \rho$.
%  
%  For~\ref{comp:trans}, suppose $a \qmMSL{\sigma \to \rho} b$ and $b \sqsubseteq c$ with $a,b,c \in \asem{\sigma_1 \to \rho}$.
%  It remains to show that $s \qmMSL{\sigma} s'$ implies $a\,s \qmMSL{\rho} c\,s'$, for all $s,s' \in \asem{\rho}$, so assume $s \qmMSL{\sigma} s'$.  
%  It follows from $a \qmMSL{\sigma \to \rho} b$ that $a\,s \qmMSL{\rho} b\,s'$.
%  Furthermore, $b \sqsubseteq c$ implies $b\,s' \sqsubseteq c\,s'$.
%  We apply the IH for $a\,s \qmMSL{\rho} c\,s'$, which proves~\ref{comp:trans}.
%  
%  For~\ref{comp:lub}, let $a \in \asem{\sigma \to \rho}$ and $A \subseteq \set{b \in \asem{\sigma \to \rho} \mid b \qmMSL{\sigma \to \rho} a}$.
%  Let $s,s' \in \asem{\sigma}$.
%  It remains to prove that $s \qmMSL{\sigma} s'$ implies $(\bigsqcup A)\,s \qmMSL{\rho} a\,s'$.
%  Because $\asem{\rho}$ is a complete lattice, $\lub A$ exists in $\asem{\rho}$ and %\changed[jj]{ is a dcpo and $\bigsqcup_{b \in A} b\,s \in \asem{\rho}$, which is true if we know $\set{b\,s \mid b \in A}$ to be a directed set (if this doesn't hold, we could prove~\ref{comp:lub} whenever ``the lub exists in the set'')}, 
%  $(\bigsqcup A)\,s = \bigsqcup_{b \in A} b\,s$.
%  Now, for all $b \in A$, $s \qmMSL{\sigma} s'$ gives us $b\,s \qmMSL{\rho} a\,s'$.
%  This implies $\bigsqcup_{b \in A} b\,s \qmMSL{\rho} a\,s'$, as required.
%\end{proof}

\begin{lemma}
  Each $\qmMSL{\gamma}$ is compatible with $\sqsubseteq$ on $\asem{\gamma}$. \jj{DONE}
\end{lemma}
%\begin{proof}
%  Consider type $\iota$.
%  Criterion~\ref{comp:trans} is immediately satisfied from the fact that $b \sqsubseteq c$ means $b = c$ for all $b,c \in \asem{\iota}$.
%  For~\ref{comp:lub}, let $a \in \asem{\iota}$ and $A \subseteq \set{b \in \asem{\iota} \mid b \qmMSL{\iota} a}$ such that $\bigsqcup A$ exists in $\asem{\iota}$.
%  Since $\asem{\iota}$ is ordered discretely wrt $\sqsubseteq$, $\lub A$ is defined only when $A$ is a singleton set.
%  Let $A = \set{b}$ such that $b \qmMSL{\iota} a$.
%  Since $b = \lub A$, it follows immediately that $\lub A \qmMSL{\iota} a$. 
%  
%  Consider type $\gamma_1 \to \gamma_2$.
%  For~\ref{comp:trans} we proceed as in the previous lemma. 
%  For~\ref{comp:lub}, let $a \in \asem{\gamma_1 \to \gamma_2}$ and $A \subseteq \set{b \in \asem{\gamma_1 \to \gamma_2} \mid b \qmMSL{\gamma_1 \to \gamma_2} a}$ such that $\lub A$ exists in $\asem{\gamma_1 \to \gamma_2}$.
%  As before, we know $A$ must be a singleton, thanks to the discrete order, so we appeal to the previous case. 
%%%  We distinguish three subcases for $A$:
%%%  \begin{itemize}
%%%    \item If $a = \bot$, then $A \subseteq \set{\bot}$.
%%%      Since $\lub A \in \asem{\iota}$, it must be that $A = \set{\bot}$ and $\lub A = a$, which implies $\lub A \qmMSL{\iota} a$.
%%%    \item If $a = \top$, then $A \subseteq \asem{\iota}$.
%%%    \item Otherwise, if $a = t$, then $A \subseteq \set{\bot, t}$.
%%%      If $A = \set{\bot}$, then $\lub A = \bot$.
%%%      Since $\bot \qmMSL{\iota} t$, the claim holds.
%%%      Otherwise, $A = \set{\bot,t}$ and $\lub A = t$, which implies $\lub A \qmMSL{\iota} a$.
%%%  \end{itemize}
%%
%%  Note that $\set{b \in \asem{\iota} \mid b \qmMSL{\iota} a}$ is a directed set wrt to $\qmMSL{\iota}$ (but not $\sqsubseteq$);
%%  if $a = \bot$ then we have $\set{\bot}$, if $a = \top$ then $\asem{\iota}$, and if $a = t$ then $\set{\bot,t}$.
%%  \jj{However, $A$ is a subset and may not be directed wrt $\sqsubseteq$, e.g. if $a = \top$ but $\top \not\in A$.
%%  
%%  We could qualify~\ref{comp:lub} by saying it holds whenever $\bigsqcup A$ exists in $\asem{\rho}$.}
%%  
%%%  We proceed as in the previous lemma, but now $\asem{\gamma_2}$ is merely a dcpo rather than a complete lattice.
%%%  This requires us to prove that $A \subseteq \set{b \in \asem{\gamma_1 \to \gamma_2} \mid b \qmMSL{\gamma_1 \to \gamma_2} a}$ is a directed set.
%%%  Since we know $\asem{\gamma_1 \to \gamma_2}$ is discretely ordered, ...
%\end{proof}

The corresponding compatibility results for $\qmH{\sigma}$ are obtained in a similar fashion.

\begin{lemma}
  \label{lem:relation_inclusion}
%  ${\sqsubseteq_\rho} \subseteq {\qmMSL{\rho}}$
%  \jj{This is too strong, because this doesn't hold for non-quasi-monotone functions;
%  e.g. negation $\sqsubseteq$ negation and negation $\qmMSL{}$ negation.}
  
  For all $f,g \in \asem{\rho}$ such that $f \sqsubseteq_\rho g$, if $f$ is quasi-monotone (i.e.~$f \qmMSL{\rho} f$) then $f \qmMSL{\rho} g$. 
  \jj{We need this on the HOCHC side instead (that's fine), o/w DONE}
\end{lemma}
%\begin{proof}
%  The relations ${\sqsubseteq_o}$ and ${\qmMSL{o}}$ coincide.
%  
%  Suppose $f \sqsubseteq_{\gamma \to \rho} g$ for some $f,g \in \asem{\gamma \to \rho}$.
%  By definition, $f\,e \sqsubseteq_{\rho} g\,e$ for all $e \in \asem{\gamma}$.
%  By the IH, $f\,e \qmMSL{\rho} g\,e$ for all $e \in \asem{\gamma}$.
%  We know that $\asem{\gamma}$ is discretely ordered by $\sqsubseteq_\gamma$, so this gives us $f \qmMSL{\gamma \to \rho} g$, as required.
%  
%  Suppose $f \sqsubseteq_{\rho' \to \rho} g$ for some $f,g \in \asem{\rho' \to \rho}$.
%  Additionally assume $f \qmMSL{\rho' \to \rho} f$.
%  As in the previous case, we obtain $f\,e \qmMSL{\rho} g\,e$ for all $e \in \asem{\rho'}$ from the IH.
%  Suppose $s \qmMSL{\rho'} s'$ for some $s,s' \in \asem{\rho'}$.  
%  Assumption $f \qmMSL{\rho' \to \rho} f$ gives us $f\,s \qmMSL{\rho} f\,s'$.
%  From $f \sqsubseteq_{\rho' \to \rho} g$ we have $f\,s' \sqsubseteq g\,s'$.
%  Finally, by~\ref{comp:trans} we have $f\,s \qmMSL{\rho} g\,s'$, which gives us $f \qmMSL{\rho' \to \rho} g$.
%\end{proof}

\subsubsection{Galois connections}

\begin{definition}
  For all predicate and constructor types $\sigma$, we construct the following functions.
  \[
    \hsem{\trSem{\sigma}} 
      \galoiS{\downToMSL{\sigma}}{\upToH{\sigma}} 
    \asem{\sigma} 
      \Galois{\downToH{\sigma}}{\upToMSL{\sigma}} 
    \hsem{\trSem{\sigma}}
  \]
  For type $\iota$:
  \[
    \upToH{\iota} \, x \defeq \left\{ \begin{array}{ll}
      \hsem{\trSem{t'}} & \text{if } \exists t':\iota.\, \asem{t'} = x \\
      x & \text{if } x = \bot \lor x = \top \\
      \top & \text{o/w}
    \end{array}\right.
    \quad
    \upToMSL{\iota} \, y \defeq \left\{ \begin{array}{ll}
      \asem{\rtSem{t}} & \text{if } \exists \rtSem{t}:\iota.\, \hsem{t} = y \\
      y & \text{if } y = \bot \lor y = \top \\
      \top & \text{o/w}
    \end{array}\right.
  \]
  \[
    \downToH{\iota} \, x \defeq \left\{ \begin{array}{ll}
      \hsem{\trSem{t'}} & \text{if } \exists t':\iota.\, \asem{t'} = x \\
      x & \text{if } x = \bot \lor x = \top \\
      \bot & \text{o/w}
    \end{array}\right.
    \quad
    \downToMSL{\iota} \, y \defeq \left\{ \begin{array}{ll}
      \asem{\rtSem{t}} & \text{if } \exists \rtSem{t}:\iota.\, \hsem{t} = y \\
      y & \text{if } y = \bot \lor y = \top \\
      \bot & \text{o/w}
    \end{array}\right.
  \]
  For type $o$, all four functions are the identity on $\asem{o} = \hsem{o}$.
  The inductive case is given by:
  \begin{align*}
    %\upToH{o}\,b &\defeq \downToH{o}\,b \defeq \upToMSL{o}\,b \defeq \downToMSL{o}\,b \defeq b \\
    \upToH{\sigma_1 \to \sigma_2}\,r &\defeq \upToH{\sigma_2} \circ r \circ \downToMSL{\sigma_1} \\
    \upToMSL{\sigma_1 \to \sigma_2}\,r &\defeq \upToMSL{\sigma_2} \circ r \circ \downToH{\sigma_1} \\
    \downToH{\sigma_1 \to \sigma_2}\,r &\defeq \downToH{\sigma_2} \circ r \circ \upToMSL{\sigma_1} \\
    \downToMSL{\sigma_1 \to \sigma_2}\,r &\defeq \downToMSL{\sigma_2} \circ r \circ \upToH{\sigma_1}
  \end{align*}
%  \jj{TODO: Define the $\rho$ cases.}
%  \[
%    \upToH{\rho} \, t \defeq \left\{ \begin{array}{ll}
%      \hsem{\trSem{t'}} & \text{if } \exists t':\rho.\, \asem{t'} = t \\
%      \topOf{\hsem{\rho}} & \text{o/w}
%    \end{array}\right.
%    \quad
%    \upToMSL{\rho} \, t' \defeq \left\{ \begin{array}{ll}
%      \asem{\rtSem{t}} & \text{if } \exists \rtSem{t}:\rho.\, \hsem{t} = t' \\
%      \topOf{\asem{\rho}} & \text{o/w}
%    \end{array}\right.
%  \]
\end{definition}

%\begin{lemma}
% For all $a \in \asem{\sigma_1 \to \sigma_2}$ and $A \subseteq \set{b \in \asem{\sigma_1 \to \sigma_2} \mid b \qmMSL{\sigma_1 \to \sigma_2} a}$ and $s \in \asem{\sigma_1}$, the set $\set{b\,s \mid b \in A}$ is directed.
% 
% $\bigsqcup_{b \in A} b\,s \in \asem{\sigma_2}$
% 
%  $\bigsqcup_{b \in A} b\,s \qmMSL{\sigma_2} a\,s'$ implies $(\bigsqcup A)\,s \qmMSL{\sigma_2} a\,s'$
%\end{lemma}
%\begin{proof}
%  If $\sigma_2 = o$, then
%  
%  For every $b \in A$, $B \subseteq \set{c \in \asem{\sigma_2} \mid c \qmMSL{\sigma_2} b\,s}$.
%  By the IH, $\bigsqcup B \qmMSL{\sigma_2} b\,s$.
%  
%  By definition, $\set{b\,s \mid b \in A} \subseteq \set{ c \in \asem{\sigma_2} \mid c \qmMSL{\sigma_1} a\,s'}$.
%  By the IH, $\bigsqcup \set{b\,s \mid b \in A} \sqsubseteq \bigsqcup \set{ c \in \asem{\sigma_2} \mid c \qmMSL{\sigma_1} a\,s'}$.
%\end{proof}

\begin{lemma}
  The above functions are quasi-monotone. \jj{DONE}
\end{lemma}
%\begin{proof}
%  \begin{description}
%    \item[Case $\iota$.]
%      Let $n,n' \in \asem{\iota}$ such that $n \qmMSL{\iota} n'$.
%      \begin{itemize}
%        \item If $n = \bot$, then $\downToH{\iota}\,n = \bot = \upToH{\iota}$.
%          Clearly, $\downToH{\iota}\,n \qmH{\iota} \downToH{\iota}\,n'$ and $\upToH{\iota}\,n \qmH{\iota} \upToH{\iota}\,n'$ regardless of $n'$.
%        \item If $n = n'$, then the claim follows from the relation $\qmH{\iota}$ including $=$.
%        \item If $n' = \top$, then we use the dual argument of $n = \bot$.
%      \end{itemize}
%      We can prove quasi-monotonicity of the remaining two functions in a completely analogous fashion, distinguishing the same three subcases for $m,m' \in \hsem{\iota}$ such that $m \qmH{\iota} m'$.
%    
%    \item[Case $o$.]
%      Immediate.
%      
%    \item[Case $\sigma_1 \to \sigma_2$.]
%      We prove one case, as the other three are analogous.
%      Let $r,r' \in \asem{\sigma_1 \to \sigma_2}$ such that $r \qmMSL{\sigma_1 \to \sigma_2} r'$.
%
%      Suppose $s \qmH{\sigma_1} s'$ for some $s,s' \in \hsem{\sigma_1}$.
%      By definition, $\upToH{\sigma_1 \to \sigma_2}\,r\,s = \upToH{\sigma_2}\,(r\,(\downToMSL{\sigma_1}\,s))$.
%      The IH gives us $\downToMSL{\sigma_1}\,s \qmMSL{\sigma_1} \downToMSL{\sigma_1}\,s'$.
%      By $r \qmMSL{\sigma_1 \to \sigma_2} r'$ we have $r\,(\downToMSL{\sigma_1}\,s)) \qmMSL{\sigma_2} r'\,(\downToMSL{\sigma_1}\,s'))$.
%      Finally, the IH proves $\upToH{\sigma_2}\,(r\,(\downToMSL{\sigma_1}\,s)) \qmH{\sigma_2} \upToH{\sigma_2}\,(r'\,(\downToMSL{\sigma_1}\,s'))$, which is $\upToH{\sigma_1 \to \sigma_2}\,r\,s \qmH{\sigma_2} \upToH{\sigma_1 \to \sigma_2}\,r'\,s'$ by definition.
%      Since this holds for all $s,s' \in \hsem{\sigma_1}$ such that $s \qmH{\sigma_1} s'$, this proves $\upToH{\sigma_1 \to \sigma_2}\,r \qmH{\sigma_1 \to \sigma_2} \upToH{\sigma_1 \to \sigma_2}\,r'\,$ and, thus, quasi-monotonicity of $\upToH{\sigma_1 \to \sigma_2}$.
%  \end{description}
%\end{proof}

\begin{corollary}
  The functions preserve quasi-monotonicity. 
  \jj{I.e.~if $t \qm t$ then $F\,t \qm F\,t$.}
\end{corollary}

\begin{lemma}
  \label{lem:type_galois}
  $\downToMSL{\sigma} \dashv \upToH{\sigma}$ and $\downToH{\sigma} \dashv \upToMSL{\sigma}$ wrt $\qm$. \jj{DONE}
\end{lemma}
%\begin{proof}
%  Consider type $\iota$.
%  \begin{align*}
%    \downToMSL{\iota}\,(\upToH{\iota}\,x) &= \left\{\begin{array}{ll}
%         \downToMSL\,(\hsem{\trSem{t'}}) = \asem{\rtSem{\trSem{t'}}} = x & \quad \text{if } x \text{ is a tree} \\
%         \downToMSL{\iota}\,x = x & \quad \text{if } x = \bot \lor x = \top \\
%         \downToMSL{\iota}\,\top = \top & \quad \text{o/w}%\\
%         %\downToMSL{\iota}\,\top = \bot & \quad \text{if } x = \top 
%      \end{array}\right. \\
%    \upToMSL{\iota}\,(\downToH{\iota}\,x) &= \left\{\begin{array}{ll}
%         \upToMSL\,(\hsem{\trSem{t'}}) = \asem{\rtSem{\trSem{t'}}} = x & \quad \text{if } x \text{ is a tree} \\
%         \upToMSL{\iota}\,x = x & \quad \text{if } x = \bot \lor x = \top \\
%         \downToMSL{\iota}\,\bot = \bot & \quad \text{o/w}%\\
%         %\upToMSL{\iota}\,\bot = \top & \quad \text{if } x = \top 
%      \end{array}\right.
%  \end{align*}
%  %The o/w cases above occur for $x = \bot$ and $x = \top$.
%  So, $\id \lesssim \downToMSL{\iota} \circ \upToH{\iota}$ and $\upToMSL{\iota} \circ \downToH{\iota} \lesssim \id$. % if $\bot \leq t \leq \top$.
%%  \jj{Otherwise, we need to drop $\top$ and the order.
%%  No, we can't drop the order, bc we need to map a wrong $t \in \hsem{\iota}$ to $\bot$ or $\top$ (only in the other direction though).
%%  How is this compatible with the discrete order on $\hsem{\iota}$?}
%  
%  \begin{align*}
%    \downToH{\iota}\,(\upToMSL{\iota}\,y) &= \left\{\begin{array}{ll}
%         \downToH{\iota}\,(\asem{\rtSem{t}}) = \hsem{\trSem{\rtSem{t}}} = y & \quad \text{if } \exists \rtSem{t}:\iota.\, \hsem{t} = y \\
%         \downToH{\iota}\,y = y  & \quad \text{if } y = \bot \lor y = \top \\
%         \downToH{\iota}\,\top = \top  & \quad \text{o/w}
%      \end{array}\right.  \\
%    \upToH{\iota}\,(\downToMSL{\iota}\,y) &= \left\{\begin{array}{ll}
%         \upToH{\iota}\,(\asem{\rtSem{t}}) = \hsem{\trSem{\rtSem{t}}} = y & \quad \text{if } \exists \rtSem{t}:\iota.\, \hsem{t} = y \\
%         %\upToH{\iota}\,(\asem{\rtSem{t}}) = \hsem{\rtSem{\trSem{t'}}} = y & \quad \text{if } \rtSem{y} \text{ is a tree no of type } \iota \\
%         %\upToH{\iota}\,\bot = \top = \bot & \quad \text{if } y = \bot \\
%         \upToH{\iota}\,y = y  & \quad \text{if } y = \bot \lor y = \top  \\
%         \upToH{\iota}\,\bot = \bot  & \quad \text{o/w}
%      \end{array}\right. 
%  \end{align*}
%  %The o/w cases above occur for $x = \bot$ and $x = \top$ as well as $y$ being a tree of the wrong type.
%  So, $\id \lesssim \downToH{\iota} \circ \upToMSL{\iota}$ and $\upToH{\iota} \circ \downToMSL{\iota} \lesssim \id$.
%  It now follows that $\downToMSL{\iota} \dashv \upToH{\iota}$ and $\downToH{\iota} \dashv \upToMSL{\iota}$.
%  
%  The claim is clear for type $o$, so consider $\sigma_1 \to \sigma_2$.
%  We show one of four parts, as it is straightforward from the IH:
%  \[
%    \upToH{\sigma_1 \to \sigma_2}\,(\downToMSL{\sigma_1 \to \sigma_2}\,r)
%      = \upToH{\sigma_1 \to \sigma_2}\,(\downToMSL{\sigma_2} \circ r \circ \upToH{\sigma_1}) 
%      = \upToH{\sigma_2} \circ \downToMSL{\sigma_2} \circ r \circ \upToH{\sigma_1} \circ \downToMSL{\sigma_1} 
%      \lesssim r 
%  \]
%\end{proof}

\begin{definition}
  We write $\canMod$ for the canonical model of $\Dhochc$ that is the limit of the ascending Kleene chain of the one-step consequence operator.
\end{definition}

\begin{definition}
  Our functions can be extended to type environments in a pointwise manner.
  Recall the HOMSL environment is $\Pi$ and the HOCHC environment $\Delta = \trSem{\Pi} \cup \mathcal{I}$ for some $\mathcal{I}$ consisting of predicates $T_\gamma$ that do not occur in $\Pi$.
  This gives rise to:
  \[
    \hsem{\trSem{\Pi}\cup \mathcal{I}} 
      \galoiS{\downToMSL{\Pi}}{\upToH{\Pi}} 
    \asem{\Pi} 
      \Galois{\downToH{\Pi}}{\upToMSL{\Pi}} 
    \hsem{\trSem{\Pi}\cup \mathcal{I}}
  \]
  where
  \begin{align*}
    \downToMSL{\Pi}(\alpha) &\defeq \prod_{x : \sigma \in \Pi} \downToMSL{\sigma}(\alpha(x)) \\
    \upToMSL{\Pi}(\alpha) &\defeq \prod_{x : \sigma \in \Pi} \upToMSL{\sigma}(\alpha(x)) \\
    \downToH{\Pi}(\beta) &\defeq \prod_{x:\sigma \in \Pi} \downToH{\sigma}(\beta(x)) \times \prod_{T_\gamma \in \mathcal{I}} \canMod(T_\gamma) \\
    \upToH{\Pi}(\beta) &\defeq \prod_{x:\sigma \in \Pi} \upToH{\sigma}(\beta(x)) \times \prod_{T_\gamma \in \mathcal{I}} \canMod(T_\gamma) 
  \end{align*}
  That is, the functions from larger-domained $\hsem{\trSem{\Pi}\cup \mathcal{I}}$ to smaller-domained $\asem{\Pi}$ are forgetful wrt to $\mathcal{I}$, while the converse functions map those extra predicates to their values in the canonical model $\canMod$ of $\Dhochc$.
  \jj{Alternatively, we could map the $T_\gamma$ to universal relations in the upwards direction (in an attempt to find a proper Galois connection at $\Pi$).
  The canonical values may not always be downwards though, or are they (when considering models specifically)?}
\end{definition}

\begin{lemma}
  \label{lem:env_maps}
  $\downToMSL{\Pi} \dashv \upToH{\Pi}$ and $\downToH{\Pi} \dashv \upToMSL{\Pi}$ wrt $\qm$. \jj{too strong, new statement:
  
  $\upToMSL{\Pi} \circ \downToH{\Pi} \lesssim \id \lesssim  \downToMSL{\Pi} \circ \upToH{\Pi}$ and 
  \[
    \upToH{\Pi} \,(\downToMSL{\Pi}\,\canMod) \lesssim \canMod \lesssim \downToH{\Pi} \,( \upToMSL{\Pi}\,\canMod)
  \]}
\end{lemma}
\begin{proof}
  It is clear from Lemma~\ref{lem:type_galois} that $\upToMSL{\Pi} \circ \downToH{\Pi} \lesssim \id \lesssim  \downToMSL{\Pi} \circ \upToH{\Pi}$ holds.
  After all, the first function adds predicates that the second one forgets about.
  
  The other pair \changed[jj]{does not hold}: 
  $\upToH{\Pi} \circ \downToMSL{\Pi} \lesssim \id \lesssim \downToH{\Pi} \circ \upToMSL{\Pi}$.
  However, we can specialise to the canonical model to obtain:
  \[
    \upToH{\Pi} \,(\downToMSL{\Pi}\,\canMod) \lesssim \canMod \lesssim \downToH{\Pi} \,( \upToMSL{\Pi}\,\canMod)
  \]
\end{proof}
%\begin{proof}
%  Consider type $\iota$.
%  \begin{align*}
%    \downToMSL{\iota}\,(\upToH{\iota}\,x) &= \left\{\begin{array}{ll}
%         \downToMSL\,(\hsem{\trSem{t'}}) = \asem{\rtSem{\trSem{t'}}} = x & \quad \text{if } x \text{ is a tree} \\
%         \downToMSL{\iota}\,x = x & \quad \text{if } x = \bot \lor x = \top \\
%         \downToMSL{\iota}\,\top = \top & \quad \text{o/w}%\\
%         %\downToMSL{\iota}\,\top = \bot & \quad \text{if } x = \top 
%      \end{array}\right. \\
%    \upToMSL{\iota}\,(\downToH{\iota}\,x) &= \left\{\begin{array}{ll}
%         \upToMSL\,(\hsem{\trSem{t'}}) = \asem{\rtSem{\trSem{t'}}} = x & \quad \text{if } x \text{ is a tree} \\
%         \upToMSL{\iota}\,x = x & \quad \text{if } x = \bot \lor x = \top \\
%         \downToMSL{\iota}\,\bot = \bot & \quad \text{o/w}%\\
%         %\upToMSL{\iota}\,\bot = \top & \quad \text{if } x = \top 
%      \end{array}\right.
%  \end{align*}
%  %The o/w cases above occur for $x = \bot$ and $x = \top$.
%  So, $\id \lesssim \downToMSL{\iota} \circ \upToH{\iota}$ and $\upToMSL{\iota} \circ \downToH{\iota} \lesssim \id$. % if $\bot \leq t \leq \top$.
%%  \jj{Otherwise, we need to drop $\top$ and the order.
%%  No, we can't drop the order, bc we need to map a wrong $t \in \hsem{\iota}$ to $\bot$ or $\top$ (only in the other direction though).
%%  How is this compatible with the discrete order on $\hsem{\iota}$?}
%  
%  \begin{align*}
%    \downToH{\iota}\,(\upToMSL{\iota}\,y) &= \left\{\begin{array}{ll}
%         \downToH{\iota}\,(\asem{\rtSem{t}}) = \hsem{\trSem{\rtSem{t}}} = y & \quad \text{if } \exists \rtSem{t}:\iota.\, \hsem{t} = y \\
%         \downToH{\iota}\,y = y  & \quad \text{if } y = \bot \lor y = \top \\
%         \downToH{\iota}\,\top = \top  & \quad \text{o/w}
%      \end{array}\right.  \\
%    \upToH{\iota}\,(\downToMSL{\iota}\,y) &= \left\{\begin{array}{ll}
%         \upToH{\iota}\,(\asem{\rtSem{t}}) = \hsem{\trSem{\rtSem{t}}} = y & \quad \text{if } \exists \rtSem{t}:\iota.\, \hsem{t} = y \\
%         %\upToH{\iota}\,(\asem{\rtSem{t}}) = \hsem{\rtSem{\trSem{t'}}} = y & \quad \text{if } \rtSem{y} \text{ is a tree no of type } \iota \\
%         %\upToH{\iota}\,\bot = \top = \bot & \quad \text{if } y = \bot \\
%         \upToH{\iota}\,y = y  & \quad \text{if } y = \bot \lor y = \top  \\
%         \upToH{\iota}\,\bot = \bot  & \quad \text{o/w}
%      \end{array}\right. 
%  \end{align*}
%  %The o/w cases above occur for $x = \bot$ and $x = \top$ as well as $y$ being a tree of the wrong type.
%  So, $\id \lesssim \downToH{\iota} \circ \upToMSL{\iota}$ and $\upToH{\iota} \circ \downToMSL{\iota} \lesssim \id$.
%  It now follows that $\downToMSL{\iota} \dashv \upToH{\iota}$ and $\downToH{\iota} \dashv \upToMSL{\iota}$.
%  
%  The claim is clear for type $o$, so consider $\sigma_1 \to \sigma_2$.
%  We show one of four parts, as it is straightforward from the IH:
%  \[
%    \upToH{\sigma_1 \to \sigma_2}\,(\downToMSL{\sigma_1 \to \sigma_2}\,r)
%      = \upToH{\sigma_1 \to \sigma_2}\,(\downToMSL{\sigma_2} \circ r \circ \upToH{\sigma_1}) 
%      = \upToH{\sigma_2} \circ \downToMSL{\sigma_2} \circ r \circ \upToH{\sigma_1} \circ \downToMSL{\sigma_1} 
%      \lesssim r 
%  \]
%\end{proof}

\jj{
The following hold at $\sigma$ (but not at $\Pi$):

$\upToH{\sigma} \circ \downToMSL{\sigma} \lesssim \id \lesssim \downToH{\sigma} \circ \upToMSL{\sigma}$

$\upToMSL{\sigma} \circ \downToH{\sigma} \lesssim \id \lesssim  \downToMSL{\sigma} \circ \upToH{\sigma}$.
}

\begin{lemma}[Inclusion of goals]
  \label{lem:goal_inclusion}
  \jj{In progress.} 
  \begin{enumerate}[label=(\roman*)]
    \item \label{incl:1}
      \[
        \upToH{\sigma}\,( \asem{G:\sigma} \,( \downToMSL{\Pi}\,\canMod)) \lesssim \hsem{\trSem{G}}(\canMod) \lesssim \downToH{\sigma}\,(  \asem{G:\sigma} \,( \upToMSL{\Pi}\,\canMod))
      \]
    \item \label{incl:2}
      \[
        \upToMSL{\sigma} \circ \hsem{\trSem{G}} \circ \downToH{\Pi} \lesssim \asem{G:\sigma} \lesssim \downToMSL{\sigma} \circ \hsem{\trSem{G}} \circ \upToH{\Pi}
      \]
  \end{enumerate}
\end{lemma}
\begin{proof}
  \jj{Continue here.}
  By induction on the structure of $M$.
  Let $\alpha \in \hsem{\trSem{\Pi} \cup \mathcal{I}}$ and $\beta \in \asem{\Pi}$.
  \jj{We need to allow extensions $\alpha$ of $\canMod$ (i.e.~$\alpha = \canMod \times \alpha'$).}
  \begin{description}
    \item[Case $M = x:\sigma$.]
      \begin{align*}
        \upToH{\sigma} \,(\asem{x:\sigma} \,( \downToMSL{\Pi}\,\canMod))
          &= \upToH{\sigma} \,((\downToMSL{\Pi}\,\canMod)\,x) \qquad \text{by sem}\\
          &= \upToH{\sigma} \,(\downToMSL{\sigma}\,(\canMod\,x)) \qquad \text{by maps}\\
          &\qm \canMod\,(x) \qquad \text{by Lem~\ref{lem:env_maps}} \\
          &= \asem{G:\sigma}(\canMod) \qquad \text{by sem}
      \end{align*}
      \begin{align*}
         \upToMSL{\sigma} \,(\hsem{\trSem{G}} \,( \downToH{\Pi}\,\beta)) 
          &= \upToMSL{\sigma} \,((\downToH{\Pi}\,\beta)\,x) \\
          &= \upToMSL{\sigma} \,(\downToH{\sigma}\,(\beta\,x)) \\
          &\qm \beta\,(x) \\
          &= \hsem{G:\sigma}(\beta)
      \end{align*}
    \item[Case $M = a : \gamma$.] \jj{Standard.}
    \item[Case $M = s\,t:\sigma$.] \jj{Standard.}
    \item[Case $M = \lambda x:\sigma_1.\,t:\sigma_2$.] \jj{Standard.}
    \item[Case $M = \truetm$.] \jj{Standard.}
    \item[Case $M = \land$.] \jj{Standard.}
    \item[Case $M = \exists x:\rho.\,G$.] \jj{TODO}
%%      \[
%%        \upToH{o} \,(\asem{\exists x:\rho.\,G} \,( \downToMSL{\Pi}\,\alpha))
%%          %= \asem{\exists x:\rho.\,G} \,( \downToMSL{\Pi}\,\alpha) \\
%%          = \max \set{\asem{G}( (\downToMSL{\Pi}\,\alpha)[x \mapsto v]) \mid v \in \asem{\rho}}
%%      \]
%      \begin{align*}
%        \upToH{o} \,(\asem{\exists x:\rho.\,G} \,( \downToMSL{\Pi}\,\canMod))
%          &= \asem{\exists x:\rho.\,G} \,( \downToMSL{\Pi}\,\canMod) \\
%          &= \max \set{\asem{G}( (\downToMSL{\Pi}\,\canMod)[x \mapsto v]) \mid v \in \asem{\rho}} \\
%          &\qm \max \set{\hsem{\trSem{G}}(\canMod[x \mapsto w]) \mid w \in \hsem{\trSem{\rho}}} \qquad \dag\\
%          &= \hsem{\exists x:\trSem{\rho}.\,\trSem{G}}(\canMod) 
%      \end{align*}
%      (\dag): We need to show that a witness $v \in \asem{\rho}$ of $\asem{G}( (\downToMSL{\Pi}\,\canMod)[x \mapsto v])$ is mapped to a witness $w \in \hsem{\trSem{\rho}}$ of $\hsem{\trSem{G}}(\canMod[x \mapsto w])$.
%      By the IH ($v \qmMSL{\rho} \downToMSL{\rho}\,(\upToH{\rho}\,v)$) and Lemma~\ref{lem:qm_goals}:
%      \begin{align*}
%        \asem{G}((\downToMSL{\Pi}\,\canMod)[x \mapsto v]) = 1
%          &\Rightarrow \asem{G}((\downToMSL{\Pi}\,\canMod)[x \mapsto \downToMSL{\rho}\,(\upToH{\rho}\,v)]) = 1 \\
%          &\Rightarrow \asem{G}(\downToMSL{\Pi}\,\canMod[x \mapsto \upToH{\rho}\,v]) = 1
%      \end{align*}
%%      For the other direction, we need to show (\ddag): 
%%      a witness $w \in \hsem{\trSem{\rho}}$ of $\hsem{\trSem{G}}(\canMod[x \mapsto w])$ maps to a witness $v \in \asem{\rho}$ of $\asem{G}( (\upToMSL{\Pi}\,\canMod)[x \mapsto v])$.
%%      By the IH ($w \qmMSL{\rho} \downToH{\rho}\,(\upToMSL{\rho}\,w)$) and Lemma~\ref{lem:qm_goals}:
%%      \begin{align*}
%%        \hsem{\trSem{G}}(\canMod[x \mapsto w]) = 1
%%          &\Rightarrow \hsem{\trSem{G}}(\canMod[x \mapsto \downToH{\rho}\,(\upToMSL{\rho}\,w)]) = 1 \\
%%          &\Rightarrow \hsem{\trSem{G}}(\canMod[x \mapsto \downToH{\rho}\,(\upToMSL{\rho}\,w)]) = 1 \\
%%      \end{align*}
      
    \item[Case $M = \exists x:\gamma.\,G$.]
      \begin{align*}
        &\upToH{o} \,(\asem{\exists x:\gamma.\,G} \,( \downToMSL{\Pi}\,\canMod)) \\
          &= \asem{\exists x:\gamma.\,G} \,( \downToMSL{\Pi}\,\canMod) \\
          &= \max \set{\asem{G}( (\downToMSL{\Pi}\,\canMod)[x \mapsto v]) \mid v \in \asem{\gamma}} \\
          &= \max \set{\asem{G}(\downToMSL{\Pi}\,\canMod[x \mapsto \upToH{\gamma}\,v]) \mid v \in \asem{\gamma}} \qquad \dag \\
          &\qm \max \set{\hsem{\trSem{G}}(\canMod[x \mapsto \upToH{\gamma}\,v]) \mid v \in \asem{\gamma}} \qquad \text{IH} \\
          %&= \max \set{\hsem{\trSem{G}}(\canMod[x \mapsto \upToH{\gamma}\,v]) \mid v \in \asem{\gamma} \land v \neq \bot} \qquad \text{by definability of $\asem{\gamma}$} \jj{???} \\
          &\qm \max \set{\hsem{\trSem{G}}(\canMod[x \mapsto w]) \mid w \in \hsem{\trSem{\gamma}} \land \exists t:\gamma.\, \hsem{\trSem{t}} = w} \quad \text{by definability of $\asem{\gamma}$} \jj{???} \\
          &= \max \set{\hsem{T_\gamma\,x \land \trSem{G}}(\canMod[x \mapsto w]) \mid w \in \hsem{\trSem{\gamma}}} \\
          &= \hsem{\trSem{\exists x:\gamma.\,G}}(\canMod) 
      \end{align*}
      (\dag): 
%      We need to show that a witness $v \in \asem{\gamma}$ of $\asem{G}( (\downToMSL{\Pi}\,\canMod)[x \mapsto v])$ is mapped to a witness $w \in \hsem{\trSem{\gamma}}$ of $\hsem{\trSem{G}}(\canMod[x \mapsto w])$.
      By the IH ($v \qmMSL{\gamma} \downToMSL{\gamma}\,(\upToH{\gamma}\,v)$) and Lemma~\ref{lem:qm_goals}:
      \begin{align*}
        \asem{G}((\downToMSL{\Pi}\,\canMod)[x \mapsto v]) = 1
          &\Rightarrow \asem{G}((\downToMSL{\Pi}\,\canMod)[x \mapsto \downToMSL{\gamma}\,(\upToH{\rho}\,v)]) = 1 \\
          &\Rightarrow \asem{G}(\downToMSL{\Pi}\,\canMod[x \mapsto \upToH{\gamma}\,v]) = 1
      \end{align*}
%      For the other direction, we need to show (\ddag): 
%      a witness $w \in \hsem{\trSem{\gamma}}$ of $\hsem{\trSem{G}}(\canMod[x \mapsto w])$ maps to a witness $v \in \asem{\rho}$ of $\asem{G}( (\upToMSL{\Pi}\,\canMod)[x \mapsto v])$.
%      By the IH ($w \qmMSL{\gamma} \downToH{\gamma}\,(\upToMSL{\gamma}\,w)$) and Lemma~\ref{lem:qm_goals}:
%      \begin{align*}
%        \hsem{\trSem{G}}(\canMod[x \mapsto w]) = 1
%          &\Rightarrow \hsem{\trSem{G}}(\canMod[x \mapsto \downToH{\gamma}\,(\upToMSL{\gamma}\,w)]) = 1 \\
%          &\Rightarrow \hsem{\trSem{G}}(\canMod[x \mapsto \downToH{\gamma}\,(\upToMSL{\gamma}\,w)]) = 1 \\
%      \end{align*}
  \end{description}
\end{proof}

\begin{lemma}
  \label{lem:qm_constants}
  $\asem{\land} \qm \asem{\land}$ and $\asem{\exists_\sigma} \qm \asem{\exists_\sigma}$. \jj{DONE}
\end{lemma}
%\begin{proof}
%  Since $\asem{\land} = (\lambda x\,y.\, \min \set{x,y}) \in \asem{o \to o \to o}$ and $\qmMSL{o}$ coincides with $\sqsubseteq_o$, $\asem{\land} \qm \asem{\land}$ holds if $\asem{\land}$ is monotone, which we know.
%  
%  The second claim is more intricate.
%  First of all, note that $\top_\rho \qmMSL{\rho} \top_\rho$ for all $\rho$, since $\top_\rho$ maps all (sets of) inputs to 1.
%  Furthermore, for all $s \in \asem{\rho}$, $s \qmMSL{\rho} \top_\rho$.
%  
%  To prove the second claim for $\sigma = \rho$, assume $r \qm r'$ for some $r,r' \in \asem{\rho \to o}$.
%  If there does not exist $s \in \asem{\rho}$ such that $r\,s =1$, then we are done, so suppose $r\,s =1$ for a specific $s \in \asem{\rho}$.
%  By the above, there exists $s' \in \asem{\rho}$ (namely $\top_\rho$) such that $s \qm s'$ and $r'\,s' = 1$, as required.
%  
%  The case for $\sigma = \gamma$ is analogous, relying on the top element of $\asem{\gamma}$ t maps all (sets of) inputs to $\top_\iota$.
%\end{proof}

\begin{lemma}[\cite{OngWagner2019} Lemma 22]
  \label{lem:qm_goals}
  If $\alpha \qmMSL{\Delta} \alpha'$, then $\asem{M:\sigma}(\alpha) \qmMSL{\sigma} \asem{M:\sigma}(\alpha')$. \jj{DONE Do we need the background theory as a variable too? For the $a:\gamma$ case? Suppose $\calA \qm \calA'$ so $c_a^{\calA} \qm c_a^{\calA'}$?}
\end{lemma}
%\begin{proof}
%  Suppose $\alpha \qmMSL{\Delta} \alpha'$. 
%  \begin{description}
%  
%    \item[Case $M = x:\sigma$.]
%      \[
%        \asem{x:\sigma}( \alpha)
%          = \alpha\,(x) 
%          \qm \alpha'\,(x) 
%          = \asem{x:\sigma}( \alpha')
%      \]
%      
%    \item[Case $M = a : \gamma$.] 
%      \[
%        \asem{a : \gamma}( \alpha)
%          = c_a^{\calA}
%          \qm c_a^{\calA}
%          = \asem{a : \gamma}(\alpha')
%      \]
%      
%    \item[Case $M = N\,N':\sigma$.] 
%      Straightforward from the IH:
%      \begin{align*}
%        \asem{N\,N':\sigma}(\alpha)
%          &= \asem{N:\sigma' \to \sigma}(\alpha)\,(\asem{N':\sigma'}(\alpha)) \\
%          &\qm \asem{N:\sigma' \to \sigma}(\alpha')\,(\asem{N':\sigma'}(\alpha')) \\
%          &= \asem{N\,N':\sigma}(\alpha')
%      \end{align*}
%      
%    \item[Case $M = \lambda x:\sigma_1.\,N:\sigma_2$.] 
%       Let $s,s' \in \asem{\sigma_1}$ such that $s \qm s'$.
%       It follows that $\alpha[x \mapsto s] \qm \alpha'[x \mapsto s']$, so the IH yields:
%      \begin{align*}
%        \asem{\lambda x:\sigma_1.\,N:\sigma_2}(\alpha)\,s
%          &= \asem{N:\sigma_2}(\alpha[x \mapsto s]) \\
%          &\qm \asem{N:\sigma_2}(\alpha'[x \mapsto s']) \\
%          &= \asem{\lambda x:\sigma_1.\,N:\sigma_2}(\alpha')\,s'
%      \end{align*}
%      Because this holds for all $s \qm s'$, the claim follows.
%      
%    \item[Case $M = \truetm$.] 
%      Immediate from $\qmMSL{o}$ coinciding with $\sqsubseteq_o$:
%      \[
%        \asem{\truetm}( \alpha)
%          = 1
%          \qm 1
%          = \asem{\truetm}(\alpha')
%      \]
%      
%    \item[Case $M = \land$.] 
%      By Lemma~\ref{lem:qm_constants}.
%    
%    \item[Case $M = \exists_\sigma$.] 
%      By Lemma~\ref{lem:qm_constants}.
%    
%  \end{description}
%\end{proof}

\begin{lemma}
  \label{lem:is_model}
  If $T' \, \beta \qmMSL{\Delta} \beta$, then $\beta$ is a model of $D$.
\end{lemma}
\begin{proof}
  \jj{???}
\end{proof}

\subsubsection{Eventual aim}

\begin{theorem}
  $D \vDash G$ implies $\Dhochc \vDash \Ghochc$
\end{theorem}
\begin{proof}
  Suppose $D \vDash G$.
  Suppose $\alpha$ be a model of $\Dhochc$.
  We obtain the following sequence of implications: \jj{It suffices to use $\alpha = \canMod$.}
  \begin{align*}
    \hsem{\Dhochc}(\alpha) = 1 
      &\Rightarrow T\,\alpha \sqsubseteq \alpha \\
      &\Rightarrow T\,\alpha \qmH{\Delta} \alpha \qquad \text{by $\sqsubseteq_\Delta$ implies $\qmH{\Delta}$ (Lem~\ref{lem:relation_inclusion}, } \alpha \text{ being the limit of the one-step operator)} \\
      &\Rightarrow \upToMSL{\Delta}\,(T\,\alpha) \qmMSL{\Delta} \upToMSL{\Delta}\,\alpha \qquad \text{by qmon of $\upToMSL{\Delta}$ (\jj{TODO})} \\
      &\Rightarrow T'\,(\upToMSL{\Delta}\,\alpha) \qmMSL{\Delta} \upToMSL{\Delta}\,\alpha \qquad \text{by inclusion lemma \jj{TODO} (Lem~\ref{lem:goal_inclusion})} \\
      &\Rightarrow \upToMSL{\Delta}\,\alpha \text{ is a model of } D \qquad \text{\jj{TODO} (Lem~\ref{lem:is_model})}\\
      &\Rightarrow \asem{G}(\upToMSL{\Delta}\,\alpha) = 1 \qquad \text{by } D \vDash G \\
      &\Rightarrow \upToMSL{o}\,(\hsem{\Ghochc}(\downToH{\Delta}\,(\upToMSL{\Delta}\,\alpha))) = 1 \qquad \text{by inclusion lemma}  \\
      &\Rightarrow \hsem{\Ghochc}(\alpha) = 1 \qquad \text{by inclusion lemma} 
  \end{align*}
  This proves $\Dhochc \vDash \Ghochc$.
\end{proof}




==> automata.tex <==
\subsection{Sorted tree automata}

We show that automaton formulas define \emph{sorted tree automata}.
In a sorted tree automaton, input symbols are sorted, not ranked (cf.~e.g.~NFTAs, see~\cite{comon1997tree});
the automaton reads higher-order constructors and accepts trees over those constructors.
The state set of a sorted tree automaton is partitioned into subsets for different sorts, which are respected by the transition relation.

Any class of automata on ranked trees gives rise to a corresponding class of automata on sorted trees that is no less expressive than the class of ranked automata.

\begin{definition}[Class of sorted tree automata]
  \label{def:gen_sorted_automaton}
   %A \emph{sorted tree automaton} is a tree automaton in which input alphabet $\Sigma$ is not ranked but \emph{sorted}.   
  For class $\class$ of automata on ranked trees, \emph{sorted $\class$} identifies a class of automata on simply sorted trees in which
   every state $q \in Q = \bigcup_{\sigma \in \sortSet} Q_\sigma$ and symbol $f \in \Sigma = \bigcup_{\sigma \in \sortSet} \Sigma_\sigma$ is associated with a single sort $\sigma \in \sortSet$, and transition relation $\transSym$ respects these sorts;
   sorted $\class$ follows the definition of $\class$ otherwise.
   
    That is, all transitions reading $f : \sigma_1 \to \dots \to \sigma_m \to \iota \in \Sigma$ must have parent states in $Q_{\sigma_{j+1} \to \dots \to \sigma_m \to \iota}$ and successor states in $Q_{\sigma_1},\dots,Q_{\sigma_j}$ (for the 1\textsuperscript{st} up to $j$\textsuperscript{th} child of $f$, resp.), for some $j \in [0..m]$ (in a top-down automaton; swap parents and successors for bottom-up).

   \jj{Is this precise yet general enough?}
\end{definition}

Although equi-expressive to NFTAs, \emph{alternating tree automata} (ATAs) achieve conciseness by allowing transitions to %a conjunction of states for the same child
conjunctions of states (see Chapter~7 in \cite{comon1997tree}).
It turns out that sorted alternating tree automata neatly capture automaton clauses.

\begin{definition}[Sorted alternating tree automaton]
  \label{def:sorted_ATA}
%   A \emph{sorted tree automaton} $\auto{}$ is a top-down tree automaton in which the alphabet $\Sigma$ is not ranked but \emph{sorted}.
%   Every state $q \in Q$ and alphabet symbol $f \in \Sigma$ is associated with a sort $\sigma \in \sortSet$, and transition relation $\transSym$ respects these sorts.

  A \emph{sorted alternating tree automaton} is a tuple $\auto{} = (Q,\Sigma,q_0,\transSym)$ where $Q = \bigcup_{\sigma \in \sortSet} Q_\sigma$ is a finite set of states, $\Sigma = \bigcup_{\sigma \in \sortSet} \Sigma_\sigma$ is a finite, sorted alphabet, $q_0 \in Q$ is the initial state, and transition set $\transSym$ is a mapping from $Q \times \Sigma$ to $\boolOf(Q \times \nats)$\footnote{$\boolOf(S)$ denotes the set of positive propositional formulas over the set of propositions $S$.} such that $\transSym$ respects sorts.
  That is, if $q \in Q_\sigma$, then:
  %\jj{We don't need $\epsilon$ to branch, but there's no reason we shouldn't allow it.}
  \[
    \transSym(q,f) \ni \left\{ \begin{array}{ll}
      \boolOf( Q_{\sigma} \times \set{1} ) & \quad \text{if } f = \epsilon \\
      \boolOf( \bigcup_{i \in [1..n]} Q_{\sigma_i} \times \set{i} ) & \quad \text{if } \exists n \geq 0.\, \exists \sigma_1,\dots,\sigma_n.\, f: \sigma_1 \to \dots \to \sigma_n \to \sigma \in \Sigma \\
      \set{\false} & \quad \text{o/w}       
    \end{array}\right.
  \]
   
   The language $\lang{\auto{}}$ of sorted ATA $\auto{}$ is defined in terms of accepting runs from the initial state, as usual for ATAs.
   However, since we are generally agnostic about the initial state, we shall, by some abuse, write $\auto{} = (Q,\Sigma,\transSym)$ for automaton family $\lambda q_0.\, (Q,\Sigma,q_0,\transSym)$ determined by $Q$, $\Sigma$, and $\transSym$.  
\end{definition}

We assume WLOG that transitions are in disjunctive normal form.
This allows us to use an NFTA-style set notation for $\transSym$, where disjunction is understood as set union.
We group conjuncts concerning the same successor node to write $\bigwedge_{j=1}^{\arity{f}} \left(\bigwedge_{k=1}^{m_{i,j}} q_{i,j,k}, \, j \right) \in \transSym(q',f)$%and even $\left(\bigwedge_{k=1}^{m_{i,1}} q_{i,1,k}, 1 \right) \land \dots \land \left(\bigwedge_{k=1}^{m_{i,\arity{f}}} q_{i,\arity{f},k}, \, \arity{f} \right) \in \transSym(q',f)$
, for all $i \in [1..n]$, whenever $\transSym(q',f) = \bigvee_{i=1}^n \bigwedge_{j=1}^{\arity{f}} \bigwedge_{k=1}^{m_{i,j}} (q_{i,j,k}, j)$.

\begin{restatable}{proposition}{eqToNFTA}
  \label{prop:eq_to_NFTA}
  Sorted alternating tree automata define the same class of languages as ordinary alternating tree automata (and, thus, NFTAs).
\end{restatable}

In fact, as long as well-sortedness is definable in class $\class$ of automata on ranked trees, then sorted $\class$ is equi-expressive to $\class$.
\jj{TODO: Check if there are other restrictions. 
Can we prove this formally? 
Is well-sortedness a safety problem? 
Do we need closure under intersection?}

Recall from Definition~\ref{def:HOMSL_intersection_type_correspondence} that an automaton formula corresponds to an intersection type system.
We use this correspondence in the next section to construct a sorted ATA that type-checks terms.
For this, we require the following two general constructions.

\begin{definition}[Product automaton and subsumption automaton]
  \label{def:gen_subsumption_automaton}
  \label{def:prod_subsumption_auto}
  \emph{Product automata} allow us to run multiple automata in parallel and are constructed as usual;
states (resp.~inputs) are tuples of states (resp.~inputs), one for each component.
We understand that input $(\epsilon, \dots, \epsilon)$ is, in fact, $\epsilon$, and write $\auto{} \times \auto{\prime}$ for the product automaton of $\auto{}$ and $\auto{\prime}$.
  NFTAs, in particular, are closed under product.
  
  They are also closed under the subsumption construction;
  an NFTA $\auto{} = (Q,\Sigma,\transSym)$ gives rise to a \emph{subsumption automaton} $\sauto{} = (\powerset{Q},\emptyset,\transSym_{\mathsf{s}})$ with:
  \begin{align*}
    \transSym_{\mathsf{s}} 
      &\defeq 
        \set{ (S, \epsilon, S \backslash \set{q_1} \cup \set{q_2}) \mid q_1 \in S \subseteq Q \land (q_2, \epsilon, q_1) \in \transSym  } \\
        &\qquad \cup \; \set{ (S_1, \epsilon, S_2) \mid S_2 \subseteq S_1 \subseteq Q}
  \end{align*}
  %\jj{We could allow the state set to be a subset of the powerset in this more general definition, but it makes the definition of the transitions messier.}
  Subsumption automaton $\sauto{}$ is a powerset automaton that reasons about the states of $\auto{}$ via $\epsilon$-transitions: 
  if there exists a path from state $S_1$ to $S_2$ in $\sauto{}$, then $\bigcap_{q \in S_1} \lang{\auto{}}(q) \subseteq \bigcap_{q \in S_2} \lang{\auto{}}(q)$.
%\jj{Not an iff!}
\end{definition}

%\jj{Musings about why we cannot preserve non-$\epsilon$-transitions:}
%For the top-down automata we are interested in, it is not possible to preserve transitions of arity greater than 1 in a powerset construction, for the same reason deterministic top-down tree automata are strictly less expressive than non-deterministic ones.
%Therefore, the subsumption construction eliminates $\Sigma$-labelled transitions.
%
%To see that this is the case, consider $\transSym = \set{ (q_a,a,\epsilon), (q_b,b,\epsilon), (q_f,f,q_a\,q_a), (q_f,f,q_b\,q_b) }$.
%The top-down tree automaton defined by this set accepts only $f\,a\,a$ and $f\,b\,b$, but a powerset construction would lose the connection between the two branches and also accept $f\,a\,b$ and $f\,b\,a$.
%This problem does not occur in a bottom-up setting, because this automaton is already bottom-up deterministic.

\subsection{Constructing the type-checking automaton}

Let $V$ be an \MSL($\omega$) automaton formula over $(\Pi,\Sigma)$, and
$\sortSet$ the set of (sub)sorts occurring in $\Sigma$.

For every $\sigma \in \sortSet$, we define an NFTA $\auto{\sigma}$ whose states are the strict types of sort $\sigma$ (equivalently, automaton clauses) and whose $\epsilon$-transitions denote subtyping (equivalently, subsumption).
These NFTAs are the sort-partitions of a larger sorted alternating tree automaton $\auto{V}$ that we call a \emph{type-checking automaton}.

Sorted ATA $\auto{V}$ accepts a term $t$ from state $\tau$ if, and only if, $t$ has strict type $\tau$ (Corollary~\ref{cor:validity_as_acceptance}).

\subsubsection{Subtyping automata $\auto{\sigma}$}

Define a degenerate NFTA $\auto{\iota} = (Q,\emptyset,\emptyset)$ with $Q \defeq \set{q_P \mid P \in \Pi}$.
Given this $\auto{\iota}$, we construct a product automaton $\auto{\sigma}$ and its subsumption automaton $\sauto{\sigma}$, for all sorts $\sigma \in \sortSet$.
By induction:
\[
  \auto{\sigma \to \sigma'} \defeq \sauto{\sigma} \times \auto{\sigma'}
    \qquad
  \sauto{\sigma \to \sigma'} \defeq \mathsf{s}(\sauto{\sigma} \times \auto{\sigma'}) 
\]

We identify states by the corresponding intersection types, using intersections for set union and arrows for products, e.g.~$q_O \land q_E \to q_O$ identifies the state $\set{(\set{q_O,q_E},q_O)}$ in $\statesA{\sauto{\iota \to \iota}} = \powerset{\powerset{\basetypes} \times \basetypes}$.

Automaton $\auto{\sigma}$ captures strict types (automaton clauses) of sort $\sigma$ with $\geq$ captured by $\epsilon$-transitions.
Automaton $\sauto{\sigma}$ captures intersection types (automaton formulas) of sort $\sigma$ with $\leq$ captured by $\epsilon$-transitions.
The inversion of the order is explained by contravariance.

\begin{restatable}[Correctness of subsumption automata]{lemma}{corrSubsumptionAutomata}
  \label{lem:correctness_subsumption_automaton}
  There exists a path $\apath{\tau}{\epsilon}{\tau'}$ in $\auto{\sigma}$, for some $\tau' \in \theta$, if and only if $\theta \leq \tau$.
\end{restatable}

\jj{TODO: We haven't technically defined $\apath{\tau}{\epsilon}{\tau'}$.}

\subsubsection{Type-checking automaton $\auto{V}$}

%Let $V$ be an \MSL($\omega$) automaton formula over $(\Pi,\Sigma)$, and
%$\sortSet$ the set of (sub)sorts occurring in $\Sigma$.
We define a \emph{type-checking (sorted alternating tree) automaton} $\auto{V} = (\states{V},\Sigma,\transSet{V})$ by:
\begin{align*}
  \states{V}    &\defeq \bigcup_{\sigma \in \sortSet } \statesA{\auto{\sigma}}\\
  %\Sigma_V     &\defeq \Sigma \\
  \transSet{V} &\defeq \bigcup_{\sigma \in \sortSet } \transSym(\auto{\sigma}) 
    \cup 
      \left\{ \left(\tau, f, \textstyle \bigvee \left\{\bigwedge_{j=1}^m (\theta_j,j) \;\middle|\; \theta_1 \to \dots \to \theta_m \to \tau \in \fromClause{\res{V}{f}} \right\} \right) 
        \;\middle|\; f \in \Sigma
      \right\}
\end{align*}
relying on $\fromClause{-}$ from Definition~\ref{def:HOMSL_intersection_type_correspondence} to map an automaton formula to the corresponding intersection type.

\begin{example}[Defining transitions from types]
  Consider some $f \in \Sigma$ and type $\tau$.
  First, note that if there do not exist types $\theta_1,\dots,\theta_m$ such that $\theta_1 \to \dots \to \theta_m \to \tau \in \fromClause{\res{V}{f}}$, then we obtain $\transSet{V}(\tau,f) = \textstyle \bigvee \emptyset = \false$.
  Otherwise, if $m = 0$, then $\transSet{V}(\tau,f) = \textstyle \bigvee \set{\bigwedge \emptyset} =\true$.

  Suppose $\fromClause{\res{V}{f}} = (q_O \land q_E \to q_U \to q_O) \land (q_O \land q_E \to q_U \to q_E) \land (q_E \to q_U \to q_E)$.
  For $m=0$, there is one non-false $f$-labelled transition for each strict type in $\fromClause{\res{V}{f}}$:
    \[
    \transSet{V}\big(q_O \land q_E \to q_U \to q_O, f \big) 
      = \transSet{V}\big(q_O \land q_E \to q_U \to q_E, f \big) 
      = \transSet{V}\big(q_E \to q_U \to q_E, f \big) 
      =  \true
  \]
  For $m=1$ and $m=2$, two strict types have matching tails, so we have only two transitions for each:
  \begin{alignat*}{4}
    \transSet{V}\big(q_U \to q_O, f \big) 
      &= (q_O \land q_E,1)
      &\transSet{V}\big(q_O, f \big) 
        &= (q_O \land q_E,1) \land (q_U,2) \\
    \transSet{V}\big(q_U \to q_E, f \big) 
      &= (q_O \land q_E,1) \lor (q_E,1) \;
      &\transSet{V}\big(q_E, f \big) 
        &= \left((q_O \land q_E,1) \land (q_U,2)\right) \lor \left((q_E,1) \land (q_U,2)\right)
\end{alignat*}
%  \begin{align*}
%      m=0 \text{ for 1\textsuperscript{st} strict type: } \quad
%        & \transSet{V}\big(q_O \land q_E \to q_U \to q_O, f \big) = \true  \\
%      m=0 \text{ for 2\textsuperscript{nd} strict type: } \quad
%        & \transSet{V}\big(q_O \land q_E \to q_U \to q_E, f \big) =  \true  \\
%      m=0 \text{ for 3\textsuperscript{rd} strict type: } \quad
%        & \transSet{V}\big(q_E \to q_U \to q_E, f \big) =  \true  \\
%      m=1 \text{ for 1\textsuperscript{st} strict type: } \quad
%        & \transSet{V}\big(q_U \to q_O, f \big) =  (q_O \land q_E,1) \\
%      m=1 \text{ for 2\textsuperscript{nd} and 3\textsuperscript{rd} strict type: } \quad
%        & \transSet{V}\big(q_U \to q_E, f \big) =  (q_O \land q_E,1) \lor (q_E,1)  \\
%      m=2 \text{ for 1\textsuperscript{st} strict type: } \quad
%        & \transSet{V}\big(q_O, f \big) =  (q_O \land q_E,1) \land (q_U,2)  \\
%      m=2 \text{ for 2\textsuperscript{nd} and 3\textsuperscript{rd} strict type: } \quad
%        & \transSet{V}\big(q_E, f \big) =  \left((q_O \land q_E,1) \land (q_U,2)\right) \lor \left((q_E,1) \land (q_U,2)\right)
%  \end{align*}
  Recall $(q_O \land q_E,1)$ is merely shorthand for $(q_O,1) \land (q_E,1)$;
  states are strict types, not intersections.
\end{example}

\begin{notation}[Run-trees]
  We write $\atree{\tau}{t}{[\theta_1,\dots,\theta_m]}{m}$ for (the existence of) a partial run of $\auto{V}$ (defined as usual for ATAs) on term $t:\sigma_1 \to \dots \to \sigma_m \to \sigma$ from state $\tau$ 
  whose unfinished branches are precisely $\bigcup_{i \in [1..m]}\set{(\tau,(n+i)) \mid \tau \in \theta_i}$, for some $n \geq 0$.
  
  Informally, such a partial run is a prefix to an accepting run on $t\,t_1 \dots t_m$ if, and only if, each $t_i$ is accepted from all states corresponding to the strict types in $\theta_i$.
  
  Formally, \emph{run-trees} are the least set closed under:
  \begin{itemize}
  
    \item $\forall \tau.\, \atree{\tau}{\epsilon}{[\tau]}{1}$
  
    \item If $(\theta_1,1) \land \dots \land (\theta_m,m) \in \transSet{V}(\tau,f)$, then $\atree{\tau}{f}{[\theta_1,\dots,\theta_m]}{m}$.
    
    \item If $\atree{\tau}{t}{[\theta_1,\dots,\theta_m]}{m}$ and $\forall \tau' \in \theta_1.\, \atree{\tau'}{t'}{[]}{0}$, then $\atree{\tau}{t\,t'}{[\theta_2,\dots,\theta_m]}{m-1}$.
    
    \item If $\atree{\tau}{t}{[\theta_1,\dots,\theta_m]}{m}$ and $\atree{\tau'}{\epsilon}{[\tau']}{1}$, then $\atree{\tau'}{t}{[\theta_1,\dots,\theta_m]}{m}$.
    
    \item If $\atree{\tau}{t}{[\theta_1,\dots,\theta_m]}{m}$ and $\parEps{[\theta_1,\dots,\theta_m]}{[\theta_1',\dots,\theta_m']}$, then $\atree{\tau}{t}{[\theta_1',\dots,\theta_m']}{m}$.
    
  \end{itemize}
  where $\parEps{[\theta_1,\dots,\theta_m]}{[\theta_1',\dots,\theta_m']}$ denotes the simultaneous $\epsilon$-transitions from (the states in) $\theta_i$ to (the states in) $\theta_i'$ defined by:
    \begin{itemize}
    
      \item If $\forall j \in [1..n].\, \atree{\tau_j}{\epsilon}{[\tau_j']}{1}$, then $\parEps{[\tau_1 \land \dots \land \tau_n]}{[\tau_1' \land \dots \land \tau_n']}$.
    
      \item If $\forall i \in [1..m].\, \parEps{[\theta_i]}{[\theta_i']}$, then $\parEps{[\theta_1,\dots,\theta_m]}{[\theta_1',\dots,\theta_m']}$.
    
  \end{itemize}
  Now, a run-tree $\atree{\tau}{t}{[]}{0}$ corresponds to an accepting run of $\auto{V}$ on $t$ from state $\tau$.
  \jj{It might be good to prove this formally if it isn't obvious.}

  For example, the following accepting run on $f\,(g\,h\,e)$ gives rise to $\atree{q_O}{f\,(g\,h\,e)}{[]}{0}$, but also $\atree{q_O}{f}{[q_E]}{1}$ and $\atree{q_E}{g}{[(\top \to q_E) \land (\top \to q_O), q_E]}{2}$ and $\atree{q_E}{g\,h}{[q_E]}{1}$, among others:
  \[
    \begin{tikzpicture}[auto,
        node distance = 8mm and 10mm,
        start chain = A going right,
        N/.style = {% nodes
            rounded corners, draw, minimum size=5mm,
            inner sep=1mm, outer sep=0mm,
            on chain=A,
            align=center},
        Acc/.style = {% accepted `nodes'
            minimum size=5mm,
            inner sep=1mm, outer sep=0mm,
            on chain=A},
        E/.style = {% edges
            arrows=->},
        every chain label/.style={inner sep=1mm, font=\footnotesize}
        ]
      \node [N] {$q_O, \epsilon$};
      \node [N] {$q_E, 1$};
      \node [N] {$(q_O \to q_E), 11$};
      \node [N] {$(\top \to q_E), 11$};
      \node [Acc] {accept};
%
      \node (B-3) [N, off chain, below=10mm of A-3.west, anchor=west] {$q_E, 12$};
      \node (B-4) [Acc, off chain, right=8 mm of B-3] {accept};
%
      \node (Z-3) [N, off chain, above=10mm of A-3.west, anchor=west] {$(q_E \to q_O), 11$};
      \node (Z-4) [N, off chain, above=10mm of A-4.west, anchor=west] {$(\top \to q_O), 11$};
      \node (Z-5) [Acc, off chain, above=10mm of A-5.west, anchor=west] {accept};
%
      \draw (A-1) edge[E] ["$f$"] (A-2)
               (A-2) edge[E] (A-3)
               (A-3) edge[E] ["$\epsilon$"] (A-4)
               (A-4) edge[E] ["$h$"] (A-5)
%
               (A-2) edge[E] (B-3)
               (A-2) edge[E] ["$g$"] (Z-3)
%
               (B-3) edge[E] ["$e$"] (B-4)
%
               (Z-3) edge[E] ["$\epsilon$"] (Z-4)
               (Z-4) edge[E] ["$h$"] (Z-5);
    \end{tikzpicture}
  \]
\end{notation}

We write $\typeSet{t}$ for $\bigwedge \set{\tau \mid \Gamma_V \vdash \hasType{t}{\tau}}$, the set of strict types of $t$, also definable by:
\[
  \typeSet{x} \defeq \Gamma_V(x)
    \qquad
  \typeSet{c} \defeq \type(c)
    \qquad 
  \typeSet{s\,t} \defeq \set{ \tau \mid \exists (\sigmaInt \to \tau) \in \typeSet{s}. \, \typeSet{t} \leq \sigmaInt}
\]
Intuitively, a term $t$ has precisely the intersection types larger than $\typeSet{t}$.

\begin{restatable}[Correctness of type-checking automaton]{lemma}{corrTypeCheckingAutomaton}
  \label{lem:corr_type-checking_automaton}
  A term $t : \sigma_1 \to \dots \to \sigma_m \to \sigma$ has type $\theta_1 \to \dots \to \theta_m \to \tau$ (i.e.~$\typeSet{t} \leq \theta_1 \to \dots \to \theta_m \to \tau$) if and only if there exists a run-tree $\atree{\tau}{t}{[\theta_1',\dots,\theta_m']}{m}$ in $\auto{V}$ with $\theta_i' \subseteq \theta_i$, for all $i \in [1..m]$.
\end{restatable}

\begin{corollary}%[Validity as acceptance]
  \label{lem:validity_as_acceptance}
  \label{cor:validity_as_acceptance}
  For every closed term $t$ and type $\tau$:
  \[
    V \vdash \toClause{\tau}{t} \rew^* \true
      \iff \Gamma_V \vdash \hasType{t}{\tau}
      \iff t \in \lang{\auto{V}}(\tau)
  \]
%  For every closed \MSL($\omega$) atom $p\,t$, the following hold:
%  \[
%    V \vdash p\,t \rew^* \true
%      \iff \Gamma_V \vdash \hasType{t}{q_{p}}
%      \iff t \in \lang{\auto{V}}(q_{p})
%  \]
\end{corollary}

%\jj{If type-checking automata are indeed just NFTAs, then we can decide satisfiability wrt HO existentials just as easily.}



==> future_work.tex <==
\section{Future Work}

As our fragment is, logically speaking, equi-expressible with model checking higher-order recursion schemes, existing model checkers algorithms from this space form a natural comparison.
More work needs to be done to draw a detailed comparison between these algorithms and our own.
Furthermore, as many of these algorithms are in their second or third generation, there will be possible optimisations that can be transfered to our own setting, in addition to novel optimisations that take advantage of our setting.

There are many possible direction in which one may wish to extend the expressive power of the fragment.
For example, a background constraint theory could be added as with HFL.
This will inevitably impact decidability but doesn't not rule out the possibility of using a related algorithm to over-approximate the problem.
